PaloBoost: An Overfitting-robust TreeBoost with Out-of-Bag Sample Regularization Techniques

Stochastic Gradient TreeBoost is often found in many winning solutions in public data science challenges. Unfortunately, the best performance requires extensive parameter tuning and can be prone to overfitting. We propose PaloBoost, a Stochastic Gradient TreeBoost model that uses novel regularization techniques to guard against overfitting and is robust to parameter settings. PaloBoost uses the under-utilized out-of-bag samples to perform gradient-aware pruning and estimate adaptive learning rates. Unlike other Stochastic Gradient TreeBoost models that use the out-of-bag samples to estimate test errors, PaloBoost treats the samples as a second batch of training samples to prune the trees and adjust the learning rates. As a result, PaloBoost can dynamically adjust tree depths and learning rates to achieve faster learning at the start and slower learning as the algorithm converges. We illustrate how these regularization techniques can be efficiently implemented and propose a new formula for calculating feature importance to reflect the node coverages and learning rates. Extensive experimental results on seven datasets demonstrate that PaloBoost is robust to overfitting, is less sensitivity to the parameters, and can also effectively identify meaningful features.

==> bk/_pb-background_v1.tex <==

\section{Background}

SGTB has its roots in Gradient Boosting Machine.
We first overview the formulation and basics of Gradient Boosting Machine (GBM), 
and then illustrate how SGTB is derived from GBM.

\subsection{Gradient Boosting Machine}

Gradient Boosting Machine (GBM) was first introduced by J. H. Friedman \cite{Friedman:2001ue}. 
Friedman discovered the connection between boosting algorithms and gradient descent algorithm in the optimization literature.
From this observation, he developed an idea that boosting is, in fact, a gradient descent algorithm at function level.   
In other words, boosting can be viewed as an iterative algorithm that tries to find the optimal ``function``, 
where the function is additively updated by fitting to the gradients (or errors) at each stage.
Under this framework, GBM generalizes various boosting algorithms - they are characterized by different loss functions e.g. logit loss for AdaBoost \cite{Freund:1999}. 

As in many machine learning algorithms, 
GBM seeks to estimate a function that minimizes the empirical risk as follows:
\begin{equation}
F^* = \argmin_F \sum_{i=1}^N L(y_i, F(\mathbf{x}_i)) \label{eq:erm}
\end{equation}
where $L(\cdot, \cdot)$ denotes a loss function, and the empirical risk is calculated over $N$ pairs of target, $y$, and input features, $\mathbf{x}$.
Frequently used loss functions are squared error, $L(y,F) = (y-F)^2$, and negative binomial log-likelihood, $L(y, F) = -yF - \log(1+e^F)$, where $y \in \{0, 1\}$.

GBM solves Equation \ref{eq:erm} by applying the gradient descent algorithm directly to the function $F$.
Its update form is as follows:
\begin{equation}
F_m(\mathbf{x}) = F_{m-1}(\mathbf{x}) + \beta_m \frac{\partial}{\partial F(\mathbf{x})} L(y, F(\mathbf{x})) \Bigr|_{F=F_{m-1}} \label{eq:gbmupdateideal}
\end{equation}
With finite data, we can only approximate the gradient term. Thus, Equation~\ref{eq:gbmupdateideal} becomes:
\begin{equation}
F_m(\mathbf{x}) = F_{m-1}(\mathbf{x}) + \beta_m h(\mathbf{x}; \mathbf{a}_m) \label{eq:gbmiter}
\end{equation}
where $h(\mathbf{x}; \mathbf{a}_m)$ is an approximation of the gradient with finite samples and $\mathbf{a}_m$ represents the parameters for the approximation function.
In GBM, $h(\mathbf{x}; \mathbf{a}_m)$ can be any parametric function such as neural net \cite{Schwenk:2000}, support vector machine \cite{Ting:2009}, and regression tree \cite{Friedman:2001ue}.
Algorithm~\ref{algo:gbm} outlines the details of GBM.

\begin{algorithm}
\DontPrintSemicolon
$F_0 = \argmin_{\beta} \sum_{i=1}^N L(y_i, \beta)$\;
\For{$m \gets 1$ \textbf{to} $M$}{
	$z_i = -\frac{\partial}{\partial F(\mathbf{x}_i)} L(y_i, F(\mathbf{x}_i)) \Bigr|_{F=F_{m-1}}$, for $i=1, \cdots, N$\;
	$\textbf{a}_m = \argmin_\textbf{a} \sum_{i=1}^N \| z_i - h(\mathbf{x}_i; \mathbf{a})\|^2$\;
	$\beta_m = \argmin_\beta \sum_{i=1}^N L(y_i, F_{m-1}(\mathbf{x}_i) + \beta h(\mathbf{x}_i; \mathbf{a}_m))$ \;
	$F_m(\mathbf{x}) = F_{m-1}(\mathbf{x}) + \beta_m h(\mathbf{x}; \mathbf{a}_m)$\;
}
\caption{Gradient Boosting Machine with Regression Tree as $h(\mathbf{x}; \mathbf{a}_m)$}
\label{algo:gbm}
\end{algorithm}

\subsection{Stochastic Gradient TreeBoost}

Stochastic Gradient TreeBoost (SGTB) improves the original GBM with two important modifications:
1) exploiting the structure of a regression tree and 2) applying subsampling at each stage.

When a regression tree is used as $h(\mathbf{x}; \mathbf{a})$, we have:
\begin{equation}
h(\mathbf{x}; \mathbf{a}) = h(\mathbf{x}; \{b_j, R_j\}_1^J) = \sum_{j=1}^J b_j \mathbbm{1}(\mathbf{x} \in R_j)
\end{equation}
where $\{R_j\}_1^J$ are disjoint regions that collectively cover the entire samples of $\mathbf{x}$, and $\{b\}_1^J$ are the estimates for $y$ for the given region.
This specific representation allows further tuning of the step size i.e. different step sizes for regions  $\beta_{jm}$ instead of a single step size per stage $\beta_m$.
We can rewrite the update form as follows:
\begin{align}
F_m(\mathbf{x}) &= F_{m-1}(\mathbf{x}) +  \sum_{j=1}^J \beta_{jm} b_j \mathbbm{1}(\mathbf{x} \in R_{jm})\\
&= F_{m-1}(\mathbf{x}) +  \sum_{j=1}^J \gamma_{jm} \mathbbm{1}(\mathbf{x} \in R_{jm})
\end{align}
where $\gamma_{jm} = \beta_{jm} b_j $.
Estimating $\gamma_{jm}$ is the same as estimating the intercept that minimizes the loss function within a disjoint region.
For example, in a regression task with a squared error, we have a closed form: 
\begin{align}
\gamma_{jm} &= \argmin_{\gamma} \sum_{\mathbf{x}_i \in R_{jm}} L(y_i, F_{m-1}(\mathbf{x}_i) + \gamma)\\
&=  \sum_{\mathbf{x}_i \in R_{jm}} (y_i -  F_{m-1}(\mathbf{x}_i) )
\end{align}
For a classification task with a negative binomial log-likelihood loss, unfortunately, we do not have a closed form solution for $\gamma$. 
In \cite{Friedman:2001ue}, Friedman suggests using a single Newton-Raphson step as the best estimate for $\gamma$ with the initial point of zero - also many other packages are implemented this way. 
Thus, the update form for $\gamma$ is:
\begin{equation}
\gamma_{jm} = \frac{\sum_{\mathbf{x}_i \in R_{jm}}(y_i - p_i)}{\sum_{\mathbf{x}_i \in R_{jm}}p_i(1-p_i)}, \text{ where } p_i = (1+e^{-F_{m-1}(\mathbf{x}_i)})^{-1}
\end{equation}

Another important modification to SGTB is subsampling, as the name Stochastic in SGTB indicates.
Motivated by the work on bagging \cite{Breiman:1996} and AdaBoost that uses random subsampling \cite{Freund:1999},
Friedman modified TreeBoost to use subsampled training samples, 
and found that this random subsampling greatly improves the performance and generalization abilities of GBM. 
Although the performance improvement varied across problems, 
he observed that this modification has greater impact on small samples with high capacity base learners.
From this observation, he postulated that the performance improvement may be due to the variance reduction as in bagging.
Algorithm~\ref{algo:treeboost} illustrates the details of SGTB with a learning rate $\nu$.
The learning rate $\nu$ is a regularization parameter that has a value between $0$ and $1$.
Lower $\nu$ values ($\le 0.1$) slow down the learning speed of SGTB and would need more iterations, 
but may achieve better generalization \cite{Friedman:2002ex}.

\begin{algorithm}
\DontPrintSemicolon
$F_0 = \argmin_{\beta} \sum_{i=1}^N L(y_i, \beta)$\;
\For{$m \gets 1$ \textbf{to} $M$}{
	$\{y_i, \mathbf{x}_i\}_1^{N^\prime} = \text{Subsample}(\{y_i, \mathbf{x}_i\}_1^{N}, \text{rate}=q)$\;
	$z_i = -\frac{\partial}{\partial F(\mathbf{x}_i)} L(y_i, F(\mathbf{x}_i)) \Bigr|_{F=F_{m-1}}$, for $i=1, \cdots, N^\prime$\;
	$\{R_{jm}\}_1^J = \text{RegressionTree}(\{z_i, \mathbf{x}_i\}_i^{N^\prime})$\;
	$\gamma_{jm} = \argmin_{\gamma} \sum_{\mathbf{x}_i \in R_{jm}} L(y_i, F_{m-1}(\mathbf{x}_i) + \gamma)$, for $j=1, \cdots, J$ \;
	$F_m(\mathbf{x}) =F_{m-1}(\mathbf{x}) +  \nu \sum_{j=1}^J \gamma_{jm} \mathbbm{1}(\mathbf{x} \in R_{jm})$\;
}
\caption{Stochastic Treeboost with Learning Rate ($\nu$)}
\label{algo:treeboost}
\end{algorithm}

SGTB is implemented in many easy-to-use open-source packages. 
Some of such implementations include Generalized Boosted Models available in \texttt{R} \cite{Ridgeway:2012wr}, TreeNet by Salford Systems \cite{treenet}, Gradient Boosting in Scikit-Learn \cite{scikit-learn}, and XGBoost implemented in \texttt{C++} \cite{Chen:2016ga}.
Although all these implement Algorithm~\ref{algo:treeboost} overall, they slightly differ in their implementation details.
For example, regarding the splitting criteria of base trees, Generalized Boosted Models uses the minimum variance criterion, Scikit-Learn uses the Friedman splitting criterion \cite{Friedman:2001ue} by default, and XGBoost uses a custom regularized splitting criterion that is obtained by greedily minimizing the Taylor approximation of the loss function \cite{Chen:2016ga}.
Moreover, they are different in treating missing values - XGBoost can handle missing values by default, while Scikit-Learn does not support.
These differences make these packages exhibit different performances even when applied to the same dataset.
However, it is generally regarded that it is difficult to claim one implementation is better than the other, 
as the performance differences are mostly specific to datasets.


==> bk/_pb-background_v2.tex <==
\section{Background}

Boosting algorithms build models in a stage-wise fashion, where the sequential learning of base learners provides a strong final model.
Breiman demonstrated that boosting can be interpreted as a gradient descent algorithm at the function level \cite{Breiman:1998ev}.
In other words, boosting is an iterative algorithm that tries to find the optimal ``function'', where the function is additively updated by fitting to the gradients (or errors) at each stage.
Later, Friedman formalized this view, and introduced Gradient Boosting Machine (GBM) that generalizes to a broad range of loss functions \cite{Friedman:2001ue}.
Stochastic Gradient Tree Boosting (SGTB) further builds on GBM to provide better predictive performance.
In this section, we provide the formulation and basics of GBM and illustrate how SGTB is derived.

\subsection{Gradient Boosting Machine}

GBM  \cite{Friedman:2001ue} seeks to estimate a function, $F^*$, that minimizes the empirical risk associated with a loss function $L(\cdot, \cdot)$ over $N$ pairs of target, $y$, and input features, $\mathbf{x}$:
\begin{equation}
F^* = \argmin_F \sum_{i=1}^N L(y_i, F(\mathbf{x}_i)) \label{eq:erm} .
\end{equation}
Examples of frequently used loss functions are squared error, $L(y,F) = (y-F)^2$ and negative binomial log-likelihood, $L(y, F) = -yF + \log(1+e^F)$, where $y \in \{0, 1\}$. 
%Under the GBM framework, the approximation function, $F(\mathbf{x})$, takes the form of a weighted sum of base learners: 
%\begin{equation}
%F(\mathbf{x}) = \sum_{i} \beta_i h_i(\mathbf{x}) \label{eq:addm},
%\end{equation}
%where $h_i(\mathbf{x})$ is a base learner and $\beta_i$ represents the corresponding weight.
GBM solves Equation \ref{eq:erm} by applying the gradient descent algorithm directly to the function $F$.
Each iterative update of the function $F$ has the form:
\begin{equation}
F_m(\mathbf{x}) = F_{m-1}(\mathbf{x}) + \beta_m \frac{\partial}{\partial F(\mathbf{x})} L(y, F(\mathbf{x})) \Bigr|_{F=F_{m-1}} \label{eq:gbmupdateideal},
\end{equation}
where $\beta_m$ is the step size.
With finite samples, we can only approximate the gradient term with an approximation function, $h(\mathbf{x})$:
%With finite samples, we can only approximate the gradient term. Thus, Equation~\ref{eq:gbmupdateideal} becomes:
\begin{equation}
F_m(\mathbf{x}) = F_{m-1}(\mathbf{x}) + \beta_m h(\mathbf{x}; \mathbf{a}_m) \label{eq:gbmiter},
\end{equation}
where $\mathbf{a}_m$ represents the parameters for the approximation function at iteration $m$.
In GBM, $h(\mathbf{x}; \mathbf{a})$ can be any parametric function such as neural net \cite{Schwenk:2000}, support vector machine \cite{Ting:2009}, and regression tree \cite{Friedman:2001ue}.
Algorithm~\ref{algo:gbm} outlines the details of GBM.

\begin{algorithm}
\DontPrintSemicolon
$F_0 = \argmin_{\beta} \sum_{i=1}^N L(y_i, \beta)$\;
\For{$m \gets 1$ \textbf{to} $M$}{
	$z_i = -\frac{\partial}{\partial F(\mathbf{x}_i)} L(y_i, F(\mathbf{x}_i)) \Bigr|_{F=F_{m-1}}$, for $i=1, \cdots, N$\;
	$\textbf{a}_m = \argmin_\textbf{a} \sum_{i=1}^N \| z_i - h(\mathbf{x}_i; \mathbf{a})\|^2$\;
	$\beta_m = \argmin_\beta \sum_{i=1}^N L(y_i, F_{m-1}(\mathbf{x}_i) + \beta h(\mathbf{x}_i; \mathbf{a}_m))$ \;
	$F_m(\mathbf{x}) = F_{m-1}(\mathbf{x}) + \beta_m h(\mathbf{x}; \mathbf{a}_m)$\;
}
\caption{Gradient Boosting Machine with Base Learner $h(\mathbf{x}; \mathbf{a})$}
\label{algo:gbm}
\end{algorithm}

An alternative perspective of GBM is to view it as an ensemble where the approximation function, $h(\mathbf{x})$, is the base learner and $\beta_m$ represents the corresponding weight.
The GBM model (outlined in Algorithm~\ref{algo:gbm}) produces a final output $F$ of the form:
\begin{equation}
F(\mathbf{x}) = F_0 + \sum_{m=1}^M \beta_m h_m(\mathbf{x}) \label{eq:addm}.
\end{equation}
In fact, XGBoost, a variant of GBM, uses this approach to develop a scalable and flexible boosting system \cite{Chen:2016ga}.
By assuming that $F$ takes the ensemble form, the optimal base learners are derived by applying Taylor approximation and a greedy optimization technique.
PaloBoost is better understood in the context of the original GBM work \cite{Friedman:2001ue}.
Thus, the notations and formulation will follow Friedman's work.

\subsection{Stochastic Gradient TreeBoost}

Stochastic Gradient TreeBoost (SGTB) introduces two important modifications to GBM: (1) tree structure aware step sizes and (2) subsampling at each stage \cite{Friedman:2001ue}.
Friedman observed that a tree partitions the input into $J$ disjoint regions ($\{R_j\}_1^J$), where each region predicts a constant value ($b_j$).
Thus, the approximation function can be expressed as:
\begin{equation}
h(\mathbf{x}; \mathbf{a}) = h(\mathbf{x}; \{b_j, R_j\}_1^J) = \sum_{j=1}^J b_j \mathbbm{1}(\mathbf{x} \in R_j).
\end{equation}
This representation allows each region to choose its own optimal step size, $\beta_{jm}$, instead of a single step size per stage $\beta_m$ to obtain a better predictive model.
Therefore, Equation \ref{eq:gbmiter} can be rewritten as:
\begin{equation}
F_m(\mathbf{x}) = F_{m-1}(\mathbf{x}) +  \sum_{j=1}^J \gamma_{jm} \mathbbm{1}(\mathbf{x} \in R_{jm})
\end{equation}
where $\gamma_{jm} = \beta_{jm} b_j $.
As a result, estimating $\gamma_{jm}$ is equivalent to estimating the intercept that minimizes the loss function within the disjoint region $R_{jm}$:
\begin{equation}
\gamma_{jm} = \argmin_{\gamma} \sum_{\mathbf{x}_i \in R_{jm}} L(y_i, F_{m-1}(\mathbf{x}_i) + \gamma).
\end{equation}

%Estimating $\gamma_{jm}$ is the same as estimating the intercept that minimizes the loss function within a disjoint region.
%For example, in a regression task with a squared error, we have a closed form: 
%\begin{align}
%\gamma_{jm} &= \argmin_{\gamma} \sum_{\mathbf{x}_i \in R_{jm}} L(y_i, F_{m-1}(\mathbf{x}_i) + \gamma)\\
%&=  \sum_{\mathbf{x}_i \in R_{jm}} (y_i -  F_{m-1}(\mathbf{x}_i) )
%\end{align}
%For a classification task with a negative binomial log-likelihood loss, unfortunately, we do not have a closed form solution for $\gamma$. 
%In \cite{Friedman:2001ue}, Friedman suggests using a single Newton-Raphson step as the best estimate for $\gamma$ with the initial point of zero - also many other packages are implemented this way. 
%Thus, the update form for $\gamma$ is:
%\begin{equation}
%\gamma_{jm} = \frac{\sum_{\mathbf{x}_i \in R_{jm}}(y_i - p_i)}{\sum_{\mathbf{x}_i \in R_{jm}}p_i(1-p_i)}, \text{ where } p_i = (1+e^{-F_{m-1}(\mathbf{x}_i)})^{-1}
%\end{equation}

The second important modification in SGTB is subsampling, which is motivated by bagging \cite{Breiman:1996}  and AdaBoost \cite{Freund:1999}.
Friedman found that random subsampling of the training samples greatly improved the performance and generalization abilities of GBM, while reducing the computing time.
Although the performance improvement varied across problems, he observed that subsampling has greater impact on small datasets with high capacity base learners.
Consequently, he postulated that the performance improvement may be due to the variance reduction as in bagging.
Typical subsampling rates ($q$) lie between 0.5 and 0.7.

However, subsampling alone maybe insufficient.
A shrinkage technique was introduced to scale the contribution of each tree by a factor $\nu$ between $0$ and $1$.
This parameter can also be viewed as the learning rate $\nu$ in the context of stochastic gradient descent.
Lower $\nu$ values ($\le 0.1$) slow down the learning speed of SGTB and would need more iterations, 
but may achieve better generalization \cite{Friedman:2002ex}.
Algorithm~\ref{algo:treeboost} illustrates the details of SGTB with a learning rate $\nu$.
Thus, SGTB has four different parameters that require tuning: (1) tree size (related to tree depth) ($J$); (2) number of trees ($M$); (3) the learning rate ($\nu$); and (4) the subsampling rate ($q$).  

\begin{algorithm}
\DontPrintSemicolon
$F_0 = \argmin_{\beta} \sum_{i=1}^N L(y_i, \beta)$\;
\For{$m \gets 1$ \textbf{to} $M$}{
	$\{y_i, \mathbf{x}_i\}_1^{N^\prime} = \text{Subsample}(\{y_i, \mathbf{x}_i\}_1^{N}, \text{rate}=q)$\;
	$z_i = -\frac{\partial}{\partial F(\mathbf{x}_i)} L(y_i, F(\mathbf{x}_i)) \Bigr|_{F=F_{m-1}}$, for $i=1, \cdots, N^\prime$\;
	$\{R_{jm}\}_1^J = \text{RegressionTree}(\{z_i, \mathbf{x}_i\}_i^{N^\prime})$\;
	$\gamma_{jm} = \argmin_{\gamma} \sum_{\mathbf{x}_i \in R_{jm}} L(y_i, F_{m-1}(\mathbf{x}_i) + \gamma)$, for $j=1, \cdots, J$ \;
	$F_m(\mathbf{x}) =F_{m-1}(\mathbf{x}) +  \nu \sum_{j=1}^J \gamma_{jm} \mathbbm{1}(\mathbf{x} \in R_{jm})$\;
}
\caption{Stochastic Treeboost with Learning Rate ($\nu$)}
\label{algo:treeboost}
\end{algorithm}

SGTB is widely available in many easy-to-use open-source packages.
Some implementations include Generalized Boosted Models available in \texttt{R} \cite{Ridgeway:2012wr}, TreeNet by Salford Systems \cite{treenet}, Gradient Boosting in Scikit-Learn \cite{scikit-learn}, and XGBoost implemented in \texttt{C++} \cite{Chen:2016ga}.
Although all packages follow Algorithm~\ref{algo:treeboost}, the implementations are slightly different.
As an example, the splitting criteria of the base learner varies across packages -- Generalized Boosted Models uses the minimum variance criterion, Scikit-Learn uses the Friedman splitting criterion \cite{Friedman:2001ue} by default, and XGBoost uses a custom regularized splitting criterion that is obtained by greedily minimizing the Taylor approximation of the loss function \cite{Chen:2016ga}.
The treatment of missing values can also differ (e.g., XGBoost can handle missing values by default, while Scikit-Learn does not support it).
Thus, the performance can vary across packages even when applied on the same dataset.
However, there is no conclusive evidence that one implementation is the best, as performance differences are dataset-dependent.


==> bk/_pb-discussions_v1.tex <==

\section{Discussions}

We introduced PaloBoost, which extends SGTB with two out-of-bag sample regularization techniques: 
1) Gradient-aware Pruning and 2) Adaptive Learning Rate.
These two regularization mechanisms are built based a new perspective on the use of out-of-bag samples. 
PaloBoost views the out-of-bag samples as another batch of training samples, 
rather than a third-party observer for tracking errors.
These regularizations enabled PaloBoost to dynamically adjust tree depths and learning rates.
Simply saying, PaloBoost almost behaves like the algorithm knows when it needs to slow down to converge. 

We outlined the details of how these regularization techniques can be implemented on top of SGTB.
Our experiments using real datasets confirmed that PaloBoost produces robust predictive performances.
Especially, when a dataset is more complex and noisy, PaloBoost more noticeably outperformed the other SGTB implementations. 
We also checked that our two regularization mechanisms worked as designed. 

Our modified feature importances showed promising results on the Friedman's Simulated Dataset.
We specifically chose the Friedman dataset, as we know the true importances of the features.
We found that the other SGTB implementations failed to identify the relevant features, 
whereas the modified feature importances of PaloBoost accurately captured the true importances.
We think that the out-of-bag sample regularizations help removing noisy nodes and features.
It would be also interesting to see if a feature selection mechanism based on our new feature importances 
can help other machine learning algorithms.

Another interesting behavior we found from the experiments is that 
there are many trees with almost zero learning rates in PaloBoost.
As their impacts are negligible,
we may be able to remove those trees without impacting the overall performance.
This may result in a much more compact sized tree boosting, while maintaining the performance. 
Perhaps, we can test if a two-steps-forward-one-step-back strategy is viable.
In other words, we can grow two or more trees, look back, and remove small learning rate trees. 
We leave these ideas for our future work.

PaloBoost is developed in the effort to make the SGTB more robust and stable. 
Although robust than the other implementations, 
it did not completely solve the issue of hyperparameter sensitivity.
We still need to specify the ``max`` learning rate and how many levels to prune.
The ideas presented in this paper are basically initial attempts for the goal.
We hope that PaloBoost can save many researchers' time and resources for tuning hyperparameters.

==> bk/_pb-experiments_v1.tex <==
\section{Experimental Results}

In this section, we verify if the Gradient-aware Pruning and Adaptive Learning Rate mechanisms are working as designed using multiple datasets.
In addition, we evaluate PaloBoost's predictive performance, comparing against three other SGTB implementations: 1) SGTB implemented using the Bonsai framework\footnote{\url{https://yubin-park.github.io/bonsai-dt/}}, 2) Scikit-Learn \cite{scikit-learn}, and 3) XGBoost \cite{Chen:2016ga}.

\subsection{Datasets and Evaluation Metrics}

Our datasets include one simulated dataset, four datasets from Kaggle \cite{kaggle}, and three datasets from the UCI repositories \cite{Dua:2017}.
Table~\ref{tab:data} lists the datasets and their basic statistics and properties.
Our benchmark study consists of three regression (labeled as REG) tasks and four classification (labeled as CLS) tasks.
The size of datasets ranges from a few thousand samples (1,994 samples) to a little bit over a million samples (114,321 samples).
We included small sample datasets, as they better highlight the sensitivity around SGTB's hyperparameters.

\begin{table}
\centering
\caption{Benchmark Datasets. For regression tasks, we list the standard deviation of the target variable, whereas the class ratios for classification tasks. The ``No. Num`` and ``No. Cat`` columns represent the number of numeric and categorical features, respectively. The ``No. Final`` column shows the final number of features after our pre-processing step.}
\label{tab:data}
\begin{tabular}{l | l | l | r | r | r | r | r} 
Dataset & Task & Missing Data & Target Stats & No. Samples & No. Num & No. Cat & No. Final  \\\hline
Friedman-Sim \cite{Friedman:1991} & REG & None & $\sigma(y)=6.953$ & 10,000 & 10 & 0 & 10  \\
Mercedes-Benz \cite{kaggle:mercedes} & REG & None & $\sigma(y)=12.67$ & 4,209 & 368 & 8 & 460 \\
Crime-Rate \cite{Redmond:2002} & REG & Present & $\sigma(y)=0.233$ & 1,994 & 126 & 1 & 127 \\
Amazon-Empl \cite{kaggle:amazon} & CLS & None & $\mu(y)=0.942 $ & 32,769 & 0 & 9 & 115 \\
Pulsar-Detect \cite{Lyon:2016, Lyon:data} & CLS & None & $\mu(y)=0.092 $ & 17,898 & 8 & 0 & 8 \\
Carvana \cite{kaggle:carvana} & CLS & Present & $\mu(y)=0.123$ & 72,983 & 17 & 14 & 151 \\
BNP-Paribas \cite{kaggle:bnp} & CLS & Present & $\mu(y)=0.761$ & 114,321 & 112 & 19 & 273 \\
\end{tabular}
\end{table}

As can be seen, many datasets have both numeric and categorical features. 
For the categorical features, we select top 20 frequent categories 
and apply one-hot encoding (also known as dummy-coding).
To keep our preprocessing minimal as possible, we applied no imputation technique.
Our SGTB implementations (including PaloBoost) and XGBoost can naturally handle missing values.
As Scikit-Learn does not support missing values, we omit Scikit-Learn for testing the datasets with missing values.

We split all datasets with a 30/70 train-test ratio i.e. 30\% for training and 70\% for test.
This specific choice of ratio is because having less training samples makes the problems more difficult and sensitive to hyperparameters.
Although we did not present in this paper, we also tried with 10/90 and 20/80 split ratios.
For those experiments, we observed that the results are often more favorable to PaloBoost. 

Our experiment steps are as follows.
PaloBoost and three other SGTB implementations are fitted to the training sets by varying max learning rates (1.0, 0.5, and 0.1).
We set the max depth of trees to be five levels - note that PaloBoost would have lower depths due to Gradient-aware Pruning.
Unless otherwise specified, we used default parameter settings for all our benchmark models.
We then apply our trained models to the test sets, and track three sets of metrics:
\begin{itemize}
\item \textbf{Predictive Performance}: We track predictive performances of all benchmark models. The performance is measured on the test sets. We use the coefficient of determination (R-squared) for the regression tasks and the Area Under the Receiver Operating Characteristic Curve (AUROC) for the classification tasks.
\item \textbf{Average Learning Rate}: This metric is only applicable for PaloBoost. Recall that PaloBoost sets different learning rates for each stage and each disjoint region of a tree. For a visualization purpose, we define the average learning rate per stage:
\begin{equation}
\bar{\nu}_m =\frac{\sum_j \nu_{jm} | R_{jm} | }{\sum_j | R_{jm} |}
\end{equation}
The average learning rate can be viewed as a weighted average of learning rates, where the weight is proportional to the leaf coverage.
We plot the average learning rate over iteration (or stage), and overlay its 20-step moving average (colored in orange).
\item \textbf{Prune Rate}: This metric is only applicable for PaloBoost. Prune Rate is defined as follows:
\begin{equation}
\text{Prune Rate} = \frac{J - J^\prime}{J}
\end{equation}
where $J$ and $J^\prime$ represent the number of disjoint regions in a tree before and after Gradient-aware Pruning, respectively.
In other words, the Prune Rate shows how many nodes are removed by the Gradient-aware Pruning mechanism.
We plot the prune rate over iteration, and overlay its 20-step moving average (colored in orange).
\end{itemize}
For Friedman's Simulated Dataset, we present a couple of additional metrics regarding the modified feature importances, 
as we know the true feature importances in this case.

\subsection{Friedman's Simulated Dataset}

We first evaluate the performance of PaloBoost using a simulated dataset, which is adopted from \cite{Friedman:1983, Friedman:1991}.
Friedman originally used this simulated dataset to test his Multidimensional Additive Spline Approximation and Multivariate Adaptive Regression Splines (MARS).
The formula for the dataset is as follows:
\begin{align}
y &= 10 \sin(\pi  x_0  x_1) + 20 (x_2-0.5)^2 + 10 x_3 + 5 x_4 + 5\epsilon \label{eq:friedman}\\
\epsilon &\sim \text{Normal}(0, 1)\\
x_i &\sim \text{Uniform}(0,1) \text{ where } i = 0 \ldots 9 
\end{align}
where $x_i$s are uniformly distributed on the interval [0,1].
For each sample, Gaussian noise $\epsilon$ with a standard deviation of five, is added.
Note that only 6 features among 10 features are used to generate the target ($y$) in Equation~\ref{eq:friedman}.
In other words, we have noisy features that i.e. features with zero importance.
We generated 10,000 samples, and trained PaloBoost and three other SGTB implementations - SGTB in Bonsai, XGBoost, and Scikit-Learn by varying learning rates (max learning rates for PaloBoost).

\begin{figure}
    \centering
        \subfloat[$R^2$, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr1.0}.pdf}}
        \subfloat[$R^2$, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr0.5}.pdf}}
        \subfloat[$R^2$, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr0.1}.pdf}}\\
        \subfloat[Avg. LR, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr1.0_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr0.5_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr0.1_avglr}.pdf}}\\
        \subfloat[Prune Rate, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr1.0_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr0.5_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr0.1_prrt}.pdf}}
        \caption{Friedman Simulated Dataset (REG). PaloBoost exhibits the best and most stable predictive performance for all learning rates. 
        			We can observe that the average learning rate is gradually and adaptively decreasing as PaloBoost iterates more. }
    \label{fig:friedman}
\end{figure}

Figure~\ref{fig:friedman} shows the predictive performance over iteration, measured in the coefficient of determination ($R^2$, the top row), average learning rate over iterations (the middle row), and prune rate over iterations (the bottom row).
As can be seen, PaloBoost exhibits the best and most stable predictive performance for all learning rate cases.
In fact, the other SGTB implementations are overfitting to the training samples, 
and show degrading performances as they iterate more. 
Even for the small learning rate of 0.1, the overfitting behaviors are apparent after 25 iterations.
On the other hand, PaloBoost shows graceful dropping of predictive performance even with high learning rates.
This behavior can be explained by looking at how the prune rate and average learning rates change over stages.
We can observe that as PaloBoost iterates, the learning rates are adaptively adjusted to smaller values, and at the same time, prune rate also goes up to make lower variance trees.

\begin{figure}
    \centering
        \includegraphics[width=1.0\textwidth]{figures/{reg_friedman_ss0.7_lr0.1_fi}.pdf}
        \caption{Feature Importances after 200 iterations. Only PaloBoost clearly identifies the irrelevant features ($x_5$ to $x_9$).
        We note that SGTB-Bonsai uses the same formula as PaloBoost. 
        This is to see if the better feature selection is due to the modified formula or PaloBoost's core algorithm.
        In this case, we conclude that both plays important roles.}
    \label{fig:feature-importance}
\end{figure}

\begin{figure}
    \centering
        \subfloat[PaloBoost]{\includegraphics[width=0.4\textwidth]{figures/{reg_friedman_ss0.7_lr0.1_fi_staged0}.pdf}}
        \subfloat[GBM]{\includegraphics[width=0.4\textwidth]{figures/{reg_friedman_ss0.7_lr0.1_fi_staged1}.pdf}}
        \caption{Feature Importances at Each Stage. We can observe how feature importances evolve over boosting stages. This plot resembles the coefficient path plot in Elastic Net \cite{Zou:2005}.}
    \label{fig:feature-importance-stage}
\end{figure}

In Section~\ref{sec:paloboost-feaures}, we introduced the modified feature importances for PaloBoost. 
Figure~\ref{fig:feature-importance} shows the modified feature importances compared against the original feature importances from the trained models.
PaloBoost clearly identifies the noisy features, while the other implementations are almost equally weighing those.
Although preliminary, this indicates PaloBoost can be also very useful for feature selection processes.
The superior performance of PaloBoost's feature selection can be explained from two folds.
First, Gradient-aware Pruning and Adaptive Learning Rates are working as designed, and removing noisy relationships.
On top of that, the modified importance formula is well capturing these dynamic attributes such as adaptive learning rates.

Figure~\ref{fig:feature-importance-stage} shows the modified feature importances over stages for the case of $\nu_{max}=0.1$.
This visualization can be viewed as somewhat analogous to the coefficient path in Elastic Net \cite{Zou:2005}.
Using this plot, we can check how feature importance values change over stages, 
and inspect the inner mechanism of PaloBoost more thoroughly.
As can be seen, the feature importances for the first six features rapidly increased till 30 iterations.
We can observe that the importances for all features slowly increase even after 30 iterations, 
but not at the sizes where they can change the order of feature importances.

\subsection{Mercedes-Benz Greener Manufacturing Dataset}

Daimler, the parent company of Mercedes-Benz, performs exhaustive tests on its pre-release cars for the safety and reliability.
The process can easily consume a substantial amount of gas and time, and generate a large volume of carbon dioxide.
In the effort to reduce the testing time and conserve the environment, 
the company released its dataset that contains various measurements (features) and time to finish the test (target) through the Kaggle platform.
The dataset has 376 features, whereas its sample size is only 4,209 - many algorithms would overfit very easily.
Thus, a predictive algorithm needs to address the curse of dimensionality \cite{Trunk:1979, Hughes:1968}.

\begin{figure*}
    \centering
        \subfloat[$R^2$, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr1.0}.pdf}}
        \subfloat[$R^2$, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.5}.pdf}}
        \subfloat[$R^2$, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.1}.pdf}} \\
        \subfloat[Avg. LR, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr1.0_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.5_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.1_avglr}.pdf}}\\
        \subfloat[Prune Rate, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr1.0_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.5_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.1_prrt}.pdf}}
        \caption{Mercedes-Benz Dataset (REG). PaloBoost outperforms the other SGTB implementations. 
        		The average learning rate for $\nu_{max}=0.1$ quickly converges to much smaller learning rates ($\approx 0.03$) after 30 iterations.}
    \label{fig:mercedes}
\end{figure*}

Figure~\ref{fig:mercedes} shows the predictive performances of all our benchmark models. 
Except for PaloBoost, all the models overfit to the training set. 
The overfitting effect is more dramatic for higher learning rate cases. 
On the other hand, PaloBoost is able to maintain its predictive performance 
even when the other models are suffering from the curse of dimensionality.
This can be explained by the average learning rate figures.
The average learning rates are adjusted to very small values after a few iterations.
Moreover, the prune rate is maintained around 40\%, meaning that almost half of nodes are removed through the Gradient-aware Prune mechanism.
We can conclude that these two mechanisms contributed to the stable performance of PaloBoost.

\subsection{Communities Crime Dataset}

Similar communities, in terms of socioeconomic and law enforcement profiles, may also experience similar types of crimes. 
Police departments can use such information to cooperate and share experience.
In the effort to make such a data-driven system, 
Redmond \cite{Redmond:2002} created a dataset by combining three data sources: US Census in 1990, US FBI Uniform Crime Report in 1995, and 1990 US Law Enforcement Management and Administrative Statistics Survey.
The dataset contains 127 features such as percent unemployed, percent under poverty, median income, etc. and a numeric target, which is violent crime rate of community.
The dataset only has 1,994 samples and even with missing values.
The curse of dimensionality is again the key challenge to address.

\begin{figure*}
    \centering
        \subfloat[$R^2$, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr1.0}.pdf}}
        \subfloat[$R^2$, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr0.5}.pdf}}
        \subfloat[$R^2$, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr0.1}.pdf}}\\
        \subfloat[Avg. LR, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr1.0_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr0.5_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr0.1_avglr}.pdf}}\\
        \subfloat[Prune Rate, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr1.0_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr0.5_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr0.1_prrt}.pdf}}
        \caption{Communities Crime Dataset (REG). Unlike the Friedman and Mercedes datasets, the predictive performances of the other models do not degrade much as they iterate more. We believe the relationship between features and target is more deterministic, and less likely to overfit. Still, PaloBoost outperforms the other models.}
    \label{fig:crime}
\end{figure*}

Figure~\ref{fig:crime} illustrates the results from the Communities Crime Dataset experiments. 
Contrary to our previous experiments, the performances of the benchmark models did not degrade as much except for the case of $\nu_{max}=1.0$.
One reason for this behavior can be found in the dataset description.
The author of the dataset stated that the dataset is carefully curated with only features that have plausible connection to crime \footnote{\url{http://archive.ics.uci.edu/ml/datasets/communities+and+crime}}.
Thus, the curse of dimensionality may not have had much significant impact on this dataset.
Yet, PaloBoost showed the most stable performances for all cases.

\subsection{Amazon Employee Access Dataset}

We now move to classification tasks.
Our first classification dataset is from Amazon.com.
Depending on their roles, Amazon's employees have different access rights on their internal web resources.
Supervisors often spend a considerable amount of time for manually granting and revoking the access rights of their employees.
To automate this manual labour and increase the overall work efficiency,
Amazon released its historical employee access dataset that contains employee attributes, resource ID, and if the access is granted or not (target).
Interestingly, the dataset has only categorical features (total 8), and by applying one-hot encoding, we obtain 115 features.

According to many top-scoring solutions on the Kaggle leaderboard, 
capturing the interaction between the categorical features seems to be critical for improving predictive performance - in other words, a highly customized preprocessing step.
In fact, this is due to the fact that the employees access rights are somewhat well defined 
given a specific configuration of employee attributes.
Thus, there exist fairly deterministic relationships between the features and the target.
However, improving the performance is not the objectives of our experiments.
As our goal is to investigate how PaloBoost performs across various datasets, 
we apply the minimal preprocessing and train our models as the same as the other experiments.

\begin{figure*}
    \centering
        \subfloat[AUROC, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr1.0}.pdf}}
        \subfloat[AUROC, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr0.5}.pdf}}
        \subfloat[AUROC, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr0.1}.pdf}}\\    
        \subfloat[Avg. LR, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr1.0_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr0.5_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr0.1_avglr}.pdf}}\\
        \subfloat[Prune Rate, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr1.0_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr0.5_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr0.1_prrt}.pdf}}
        \caption{Amazon Employee Access Dataset (CLS). 
        	PaloBoost is slower to converge, showing poorer performance than the other models. 
        We believe the dataset is less likely to overfit. 
        In fact, higher learning rates provide comparable (or better) performance with lower learning rates for all models.}
    \label{fig:amazon}
\end{figure*}

Figure~\ref{fig:amazon} presents the results from the Amazon Employee Dataset experiment.
In this experiment, we see a somewhat different pattern in the predictive performance graphs.
Except for the Scikit-Learn model, the performances of all models are still improving in 200 iterations.
In other words, these models have not converged yet.
We can think of two reasons for this behavior. 
First, all features in this dataset are categorical, so the degree of freedom in the input space is finite - 
less of the curse of dimensionality.
Second, there exist fairly deterministic relationships between the features and the target.
These two factors would make the models less overfit to the training samples.

Another important aspect of this experiment is that PaloBoost converged slower than the other models.
This is because PaloBoost has two additional regularization mechanisms. 
These regularizations would positively impact the performance if the problem is complex enough e.g. easy to overfit, large amount of noise, etc.
However, in this case, the SGTB models without the regularizations seem to work fine, 
thus the regularizations are, in fact, hurting the PaloBoost's performance.

\subsection{Pulsar Detection Dataset}

Pulsars, rapidly rotating neutron stars, are known to emit a detectable pattern of electromagnetic radiation.
However, due to radio frequency interference and noise, automated detection based on the pattern is often a non-trivial task.
Nowadays, machine learning techniques are adopted to extract candidates for detecting pulsars.
In the effort to develop such machine learning detection algorithms, 
Lyon curated and published the HTRU2 (High Time Resolution Universe Survey - South) dataset \cite{Lyon:2016, Lyon:data}.
The dataset contains the profiles of electromagnetic waves and the label (pulsar or not) of 17,898 examples, 
where 1,639 examples are pulsars (positive class). 
All features are numeric and have no missing values.

\begin{figure*}
    \centering
        \subfloat[AUROC, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr1.0}.pdf}}
        \subfloat[AUROC, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr0.5}.pdf}}
        \subfloat[AUROC, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr0.1}.pdf}}\\
        \subfloat[Avg. LR, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr1.0_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr0.5_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr0.1_avglr}.pdf}}\\
        \subfloat[Prune Rate, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr1.0_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr0.5_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr0.1_prrt}.pdf}}
        \caption{Pulsar Detection Dataset [CLS]. PaloBoost exhibits the most stable performances. 
        		AUROC values are overall very high, indicating the problem is relatively easy.
		However, the other models quickly overfit to the training samples when their learning rates are high.}
    \label{fig:pulsar}
\end{figure*}

Figure~\ref{fig:pulsar} illustrates the results from the Pulsar Detection Dataset experiment.
As can be seen, PaloBoost exhibits the most stable and best performance overall.
However, the performance differences are practically indistinguishable for smaller learning rates.
A reason for this behavior can be found in how the dataset is curated.
The author of the dataset curated only engineered features that are strongly correlated with the target variable.
Even a single, although custom, decision tree algorithm could achieve a reasonable performance \cite{Lyon:2016}. 
In other words, the dataset has no noisy features, thus overfitting is less likely to happen even for complex models.

\subsection{Carvana Dataset}

When auto dealers purchase used cars from an auction, 
there is a risk of purchasing cars with serious issues such as tampered odometers and mechanical issues, 
which is commonly referred as ``kicks`` in the industry.
Carvana is an online used-car dealers company. 
The company released its dataset that contains used cars' attributes, such as make, model, vehicle age, odometer, etc., and the target variable (kick or not). 
The dataset has 72,983 samples. 
Its 14 categorical and 17 numeric features are converted into 151 numeric features after our preprocessing step.
As the dataset has missing values, we omit Scikit-Learn from our benchmark.

\begin{figure*}
    \centering
        \subfloat[AUROC, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr1.0}.pdf}}
        \subfloat[AUROC, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr0.5}.pdf}}
        \subfloat[AUROC, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr0.1}.pdf}}\\    
        \subfloat[Avg. LR, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr1.0_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr0.5_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr0.1_avglr}.pdf}}\\
        \subfloat[Prune Rate, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr1.0_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr0.5_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr0.1_prrt}.pdf}}
        \caption{Carvana Dataset [CLS]. PaloBoost does not show any performance degradation even for higher learning rates. 
        The other models show overfitting behaviors even for smaller learning rates. 
        The average learning rates for PaloBoost nicely attenuates as PaloBoost iterates, preventing the algorithm to overfit. }
    \label{fig:carvana}
\end{figure*}

Figure~\ref{fig:carvana} shows the results from the dataset.
As can be seen, the benchmark models clearly show overfitting behaviors for all cases.
Even on the Kaggle's public and private leaderboards\footnote{Kaggle sets one third of test data for ranking the public leaderboard, and the rest for the private leaderboard. The private leaderboard is closed during the competition, and announced after the competition is closed. This is to prevent the overfitting on the test set \cite{Blum:2015}.}, 
there has been a shake-up in the top ranks most likely due to overfitting. 
In other words, the dataset is easy to overfit as shown on both the Kaggle and our experiment examples.
Notably, PaloBoost exhibits extremely stable predictive performances, recording the best scores for all cases.
We can also observe that the Gradient-aware Pruning and Adaptive Learning Rate mechanisms are working as designed - adaptively pruning leaves and lowering the learning rates.

\subsection{BNP Paribas Cardif Claims Dataset}

Insurance claim payments involve many levels of manual checks, sometimes requires more information to be collected, 
and can take a substantial amount of time till the final payments.
Some of these claims, however, can be processed much faster with machine learning techniques.
BNP Paribas Cardif, one of the largest personal insurance company, released some of its data via the Kaggle platform
that contains various claim attributes (features) and if the claim's approval could be accelerated or not (target).
The dataset consists of 114,321 samples. 
Its 19 categorical and 112 numeric features are converted into 273 numeric features after our preprocessing step.
As the dataset has many missing values, we omit Scikit-Learn from our benchmark.
This dataset is the largest dataset in our benchmark study, and shows a fair degree of complexity. 

\begin{figure*}
    \centering
        \subfloat[AUROC, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr1.0}.pdf}}
        \subfloat[AUROC, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr0.5}.pdf}}
        \subfloat[AUROC, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr0.1}.pdf}}\\
        \subfloat[Avg. LR, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr1.0_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr0.5_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr0.1_avglr}.pdf}}\\
        \subfloat[Prune Rate, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr1.0_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr0.5_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr0.1_prrt}.pdf}}
        \caption{BNP-Paribas Cardif Dataset [CLS]. For higher learning rates, even PaloBoost shows some degree of overfitting, however, the level of performance degradation is much less than the other models.
        The average learning rates for PaloBoost adaptively decrease over iterations.
        PaloBoost shows the best and stable performances for all cases.}
    \label{fig:bnp}
\end{figure*}

Figure~\ref{fig:bnp} illustrates the results from the BNP Paribas Cardif Claims Dataset experiment.
As can be seen, PaloBoost shows the most stable and best predictive performances for all cases. 
Thus far in our experiments, we have observed that PaloBoost outperforms regular SGTB models 
when a dataset has many noisy features and easy to overfit.
The results from this experiment also adds an additional evidence to our finding.
The competitors involved in this Kaggle challenge remarked that they suspect the dataset has additional noise to the features\footnote{\url{https://www.kaggle.com/c/bnp-paribas-cardif-claims-management/discussion/19240}, \\\url{https://www.kaggle.com/c/bnp-paribas-cardif-claims-management/discussion/20247}, and some more in the Kaggle discussion board.}.
Many winning solutions were based on extensive feature engineerings, identifying the relationships of the features, and removing the noisy features.
Recall the experimental results on the modified feature importances using the Friedman Simulated Dataset.
In that experiment, PaloBoost could effectively identify noisy features, while other SGTB implementations were not able to.
This may explain why PaloBoost can outperform other SGTB implementations when a minimal preprocessing is applied to a noisy dataset.















==> bk/_pb-experiments_v2.tex <==
\section{Experimental Results}

PaloBoost is implemented on Python using the Bonsai Decision Tree framework \cite{bonsai-dt}, which allows easy manipulation of decision trees.
The Bonsai framework is mostly written in Python with its core computation modules written in Cython, to provide C-like performance.
Our implementation of PaloBoost is made publicly available as an extension to Bonsai.

PaloBoost is evaluated on a variety of datasets (simulated and real-world) and compared against state-of-the-art implementations.
In this section, we will analyze the following aspects of PaloBoost:
\begin{itemize}
\item How different are the learning rates and tree depths at each individual stage?
\item How sensitive is PaloBoost to the specified hyperparameters?
\item How does the predictive performance compare with other SGTB implementations?
\item Is PaloBoost more computationally expensive than existing SGTB implementations?
\end{itemize}
All experiments are carried out on a single machine running macOS High Sierra 10.13.6 with 2.7 GHz Intel Core i5 CPU and 8 GB of RAM.


\subsection{Datasets}

Seven different datasets are used to evaluate the SGTB variants, including PaloBoost.
We use one simulated dataset and six publicly available datasets, two from the UC Irvine (UCI) machine learning repository \cite{Dua:2017} and four from Kaggle \cite{kaggle}, a popular data science competition platform.
Our benchmark study consists of three regression tasks and four classification tasks.
The sizes of the datasets range from a few thousand samples (1,994 samples) to a little bit over a hundred thousand samples (114,321 samples).
Small datasets are included to highlight the performance sensitivity with respect to the hyperparameters.
Table \ref{tab:data} lists the seven real-world datasets and their associated characteristics.
A brief overview of each dataset will be provided in the context of their respective tasks.

\begin{table}
\centering
\caption{Benchmark Datasets. For regression tasks, we list the standard deviation of the target variable, whereas the class ratios for classification tasks. The ``\# Real'' and ``\# Cat'' columns represent the number of numeric and categorical features, respectively. The ``\# Final'' column shows the final number of features after our pre-processing step.}
\label{tab:data}
\begin{tabular}{l  l   l   r   r   r   r   r} 
\toprule
Dataset & Task & Missing Data & Target Stats & \# Samples & \# Real & \# Cat & \# Final  \\
\midrule
Friedman-Sim \cite{Friedman:1991} & REG & None & $\sigma(y)=6.953$ & 10,000 & 10 & 0 & 10  \\
Mercedes-Benz \cite{kaggle:mercedes} & REG & None & $\sigma(y)=12.67$ & 4,209 & 368 & 8 & 460 \\
Crime-Rate \cite{Redmond:2002} & REG & Present & $\sigma(y)=0.233$ & 1,994 & 126 & 1 & 127 \\
Amazon-Empl \cite{kaggle:amazon} & CLS & None & $\mu(y)=0.942 $ & 32,769 & 0 & 9 & 115 \\
Pulsar-Detect \cite{Lyon:2016, Lyon:data} & CLS & None & $\mu(y)=0.092 $ & 17,898 & 8 & 0 & 8 \\
Carvana \cite{kaggle:carvana} & CLS & Present & $\mu(y)=0.123$ & 72,983 & 17 & 14 & 151 \\
BNP-Paribas \cite{kaggle:bnp} & CLS & Present & $\mu(y)=0.761$ & 114,321 & 112 & 19 & 273 \\
\bottomrule
\end{tabular}
\end{table}

Many of the datasets contain both numeric and categorical features.
For the categorical features, the top 20 frequent categories are selected and transformed using one-hot encoding (also known as dummy-coding).
To minimize the impact of preprocessing, no additional techniques were applied (e.g. imputation, outlier detection).
While XGBoost and our SGTB implementations (including PaloBoost) can naturally handle missing values, we omit Scikit-Learn for datasets with missing values as it does not support missing values.

\subsection{Baselines}

We compare PaloBoost with three other baseline models as follows:
\begin{itemize}
\item Scikit-Learn \cite{scikit-learn}, the de-facto machine learning library in Python that has been widely adopted.
\item XGBoost \cite{Chen:2016ga}, the battle-tested library that has won many data science challenges.
\item Bonsai-SGTB, an SGTB implementation using the Bonsai framework \footnote{\url{https://yubin-park.github.io/bonsai-dt/}}.
\end{itemize}
While there are many newly developed SGTB implementations (e.g., LightGBM, CatBoost), they are not included in our study for several reasons.
First, we observed that the overfitting behavior of these packages are similar to the Scikit-Learn and XGBoost as they focus primarily on implementation details and feature engineering.
CatBoost focuses on more efficiently encoding categorical variables using Target-based Statistics and permutation techniques \cite{Prokhorenkova:2017ul, Dorogush:2017vz}.
LightGBM primarily focuses on training speed using less memory in distributed settings \cite{Ke:2017ut}. 
Secondly, our objective is to characterize the behaviors of the two regularization techniques in PaloBoost, rather than to claim that PaloBoost outperforms other SGTB implementations.
We note that our regularization techniques, Gradient-aware Pruning and Adaptive Learning Rate, can be added to any existing SGTB implementations.
Therefore, the three baseline models serve as suitable representations for other implementations.


%This is because they focus mostly on the implementation and feature engineering.
%For example, CatBoost focuses on more efficiently encoding categorical variables using Traget-based Statistics and permutation techniques \cite{Prokhorenkova:2017ul, Dorogush:2017vz}.
%LightGBM primarily focuses on training speed using less memory in distributed settings \cite{Ke:2017ut}. 
%Although, LightGBM grows its base learner tree with the best-first approach rather than the depth-first approach,  
%the hyperparameter tuning for these packages, learning rate and max depth (max leaves for LightGBM), still remains the same as a regular SGTB. 


%There are many newly developed SGTB implementations such as LightGBM and CatBoost.
%However, we did not include them in our baseline for two reasons.
%First, we observed that the overfitting behaviors of these packages are not much different from a regular SGTB implementation. 
%This is because they focus mostly on the implementation and feature engineering.
%For example, CatBoost focuses on more efficiently encoding categorical variables using Traget-based Statistics and permutation techniques \cite{Prokhorenkova:2017ul, Dorogush:2017vz}.
%LightGBM primarily focuses on training speed using less memory in distributed settings \cite{Ke:2017ut}. 
%Although, LightGBM grows its base learner tree with the best-first approach rather than the depth-first approach,  
%the hyperparameter tuning for these packages, learning rate and max depth (max leaves for LightGBM), still remains the same as a regular SGTB. 
%Secondly, our objective is to characterize the behaviors of the two regularization techniques in PaloBoost, rather than to claim that PaloBoost outperforms other SGTB implementations.
%Note that the two regularization techniques, Gradient-aware Pruning and Adaptive Learning Rate, can also be added to any existing SGTB implementations with minor modifications of the source codes. 
%In short, we concluded that our two baseline models are representative enough for other implementations, 
%and they can effectively highlight the characteristics of PaloBoost without cluttering the graphs.


\subsection{Setup \& Evaluation Metrics}

%Each dataset is split into a 
All datasets are split with a 30/70 train-test ratio (i.e., 30\% for training and 70\% for test). 
While we performed extensive experiments using other ratio choices and found similar behaviors, this specific choice showcases the sensitivity of SGTB to hyperparameters.
With larger training ratios (e.g., 50/50, 60/40, 70/30, 80/20), we found that it was difficult to visualize the overfitting behaviors for many of the baseline models.
On the contrary, for smaller training ratios such as 10/90 and 20/80, the results were significantly more favorable to PaloBoost.
The 30/70 split best illustrated the characteristics of PaloBoost without significantly sacrificing the training sample size.

For each SGTB implementation, we tested three different learning rates that spanned the spectrum for $\nu$ (1.0, 0.5, and 0.1).
Also for consistency across the models, the tree depth was set to be five levels (note that PaloBoost will have lower depths due to Gradient-aware pruning).
Unless otherwise specified, default parameter settings were used for all our benchmark models.
The trained models (on the 30\% training set) are then applied to the test set where we track the predictive performance.
This is measured using the coefficient of determination ($R^2$) and the Area Under the Receiver Operating Characteristic Curve (AUROC) for the regression and classification tasks, respectively.
We also track two different metrics for PaloBoost:
\begin{itemize}
\item \textbf{Average Learning Rate}:
For visualization purposes, we defined the average learning rate per stage to compress the different learning rates for each disjoint region of a tree.
This is a weighted average of the learning rates, where the weights are proportional to the leaf coverage, and is defined as:
\begin{equation}
\bar{\nu}_m =\frac{\sum_j \nu_{jm} | R_{jm} | }{\sum_j | R_{jm} |}
\end{equation}
\item \textbf{Prune Rate}: We measure the number of nodes removed by the Gradient-aware pruning mechanism.
The prune rate is defined as follows:
\begin{equation}
\text{Prune Rate} = \frac{J - J^\prime}{J}
\end{equation}
where $J$ and $J^\prime$ represent the number of disjoint regions in a tree before and after Gradient-aware Pruning, respectively.
%In other words, the Prune Rate shows how many nodes are removed by the Gradient-aware Pruning mechanism.
%We plot the prune rate over iteration, and overlay its 20-step moving average (colored in orange).
\end{itemize}

\subsection{Simulated Dataset}

\emph{Description}. The simulated dataset is adopted from Friedman \cite{Friedman:1983, Friedman:1991}, to introduce noisy features (i.e., features with zero importance).
The formula for the dataset is as follows:
\begin{align}
y &= 10 \sin(\pi  x_0  x_1) + 20 (x_2-0.5)^2 + 10 x_3 + 5 x_4 + 5\epsilon \label{eq:friedman}\\
\epsilon &\sim \text{Normal}(0, 1)\\
x_i &\sim \text{Uniform}(0,1) \text{ where } i = 0 \ldots 9 
\end{align}
where $x_i$s are uniformly distributed on the interval [0,1].
For each sample, Gaussian noise $\epsilon$ with a standard deviation of five, is added.
Note that only 5 features among 10 features ($x_0 - x_4$) are used to generate the target ($y$) in Equation~\ref{eq:friedman}.
Our simulated dataset contains 10,000 samples.

\begin{figure}[tb]
    \centering
        \subfloat[$R^2$, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr1.0}.pdf}}
        \subfloat[$R^2$, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr0.5}.pdf}}
        \subfloat[$R^2$, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr0.1}.pdf}}\\
        \caption{Predictive performance on the Simulated Dataset.}
    \label{fig:friedman-perf}
\end{figure}

\emph{Predictive Performance}. Figure \ref{fig:friedman-perf} shows the coefficient of determination ($R^2$) over the iteration for the three different learning rates.
PaloBoost exhibits the best and most stable predictive performance for all the learning rates.
While the other SGTB implementations show a significant degradation in predictive performance as they iterate more, PaloBoost displays a graceful drop of predictive performance even with high learning rates.
Even for a small learning rate of 0.1, the overfitting behavior of SGTB becomes apparent after 25 iterations.
Moreover, the predictive performance of PaloBoost varies considerably less across the three different learning rates, illustrating better robustness to the parameter setting ($\nu_{max}$).


\emph{Average Learning Rate and Prune Rate}.
The gradual decline of predictive performance in PaloBoost can be better understood by analyzing the prune rate and average learning rate at each stage.
Figure \ref{fig:friedman-palo} displays the average learning rate (top row) and the prune rate (bottom row) over the same iterations.
We also overlay the 20-step moving average (colored in orange), to visualize the overall trend.
As can be seen, the learning rate for each stage is quite different, and often below the specified maximum rate.
We can also observe that as the number of stages increases, the learning rates are adaptively adjusting to smaller values (more noticeable in $\nu_{max} = 0.1$).
In addition, the prune rate increases to yield lower variance trees.
Thus, the two regularization mechanisms serve as a guard against overfitting.

\begin{figure}[tb]
\centering
        \subfloat[Avg. LR, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr1.0_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr0.5_avglr}.pdf}}
        \subfloat[Avg. LR, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr0.1_avglr}.pdf}}\\
        \subfloat[Prune Rate, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr1.0_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr0.5_prrt}.pdf}}
        \subfloat[Prune Rate, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_friedman_ss0.7_lr0.1_prrt}.pdf}}
                \caption{The average learning rate and prune rate for PaloBoost on the Simulated Dataset.}
    \label{fig:friedman-palo}
\end{figure}


\emph{Computational Speed}.
Gradient-aware pruning and adaptive learning add computational complexity to SGTB. 
To determine the impact of our modifications, we measured the training speeds of the four SGTB models (PaloBoost, Bonsai-SGTB, Scikit-learn, and XGBoost). 
Figure~\ref{fig:speed} shows the measured training time over simulated training sample sizes.
As can be seen, the performance of PaloBoost is comparable with the other implementations even for large sample sizes (e.g. one million samples).
While PaloBoost is marginally slower than SGTB-Bonsai, the two regularization techniques do not slow down the overall training process much.

\begin{figure}
    \centering
        \includegraphics[width=0.6\columnwidth]{figures/{reg_friedman_ss0.7_lr0.1_speed}.pdf}
        \caption{Runtime experiment on a macOS High Sierra 10.13.6 machine with 2.7 GHz Intel Core i5 CPU, Python 2.7.14, Scikit-Learn 0.19.1, and XGBoost 0.6.}
    \label{fig:speed}
\end{figure}



\begin{figure}
    \centering
        \includegraphics[width=1.0\textwidth]{figures/{reg_friedman_ss0.7_lr0.1_fi}.pdf}
        \caption{The feature importances after 200 iterations. Only the first five features, $x_0$ to $x_4$, are used to generate the target.}
       %Only PaloBoost clearly identifies the irrelevant features ($x_5$ to $x_9$).
        %We note that SGTB-Bonsai uses the same formula as PaloBoost.}
    \label{fig:feature-importance}
\end{figure}

\begin{figure}
    \centering
            \includegraphics[width=0.6\textwidth]{figures/{reg_friedman_ss0.7_lr0.1_fi_staged0}.pdf}

       %\subfloat[PaloBoost]{\includegraphics[width=0.4\textwidth]{figures/{reg_friedman_ss0.7_lr0.1_fi_staged0}.pdf}}
        %\subfloat[GBM]{\includegraphics[width=0.4\textwidth]{figures/{reg_friedman_ss0.7_lr0.1_fi_staged1}.pdf}}
        \caption{The evolution of feature importances at each stage of PaloBoost. This plot resembles the coefficient path plot in Elastic Net \cite{Zou:2005}.}
    \label{fig:feature-importance-stage}
\end{figure}

\emph{Feature Importance}.
Since the dataset is simulated, the true feature importance is known, with only 5 features ($x_0 - x_4$) used to generate the target.
We compared the feature importances from the four different trained models with 200 iterations ($M=200$) and a learning rate of 0.1 ($\nu_{max}=0.1$).
PaloBoost and SGTB-Bonsai use the proposed feature importance formula (see Section \ref{sec:paloboost-feaures}), while XGBoost and Scikit-Learn use the standard feature importance formula (summation of the squared error improvements per feature).
Figure~\ref{fig:feature-importance} shows the feature importances from all four SGTB models\footnote{The results are similar for $M=50$ but less dramatic.}.
PaloBoost clearly identifies the noisy features ($x_5-x_9$), while XGBoost and Scikit-Learn estimate similar importances between the relevant and noisy features.
Although preliminary, this indicates PaloBoost can be also very useful for the feature selection processes.

The superiority of PaloBoost's feature importance is likely due to two different aspects.
First, gradient-aware pruning and adaptive learning rates are removing noisy features, as regions that do not generalize well are either pruned or have a small adaptive learning rate.
Secondly, the modified importance formula encapsulates the learning rate, coverage, and impact of the feature, using the leaf-centric multiplicative factor $|R_{jm}| \nu_{jm} |\gamma_{jm}|$.
This can be confirmed in Figure \ref{fig:feature-importance} by comparing the importance estimates for features $x_5-x_9$ between SGTB-Bonsai and XGBoost (or Scikit-Learn).
SGTB-Bonsai uses the proposed feature importance formula with the same learning rate ($nu_{jm} = 0.1$), yet still identifies lower importance values for $x_5-x_9$.
While accounting for the region size ($|R_{jm}|$) and node estimate ($\gamma_{jm}$) is clearly important, the adaptive learning rate provides further separation of the noisy features.
Thus, we conclude that both aspects play important roles for the superior performance.

We further explored PaloBoost's feature importance estimates as a function of the iterations for the same learning rate ($\nu_{max}=0.1$).
Figure~\ref{fig:feature-importance-stage} visualizes the evolution of the feature importance estimates and offers a perspective analogous to the coefficient path in Elastic Net \cite{Zou:2005}.
Using this plot, we can inspect the inner mechanism of PaloBoost more thoroughly.
As can be seen, the feature importances for the first five features rapidly increases through the first 30 iterations, after which they slowly increase.
Moreover, after 20 iterations, the order of the features no longer change and reflect the true feature rank.
We also note that this visualization can also be used to determine the stopping criteria for the number of iterations.


\begin{figure*}
    \centering
        \subfloat[Mercedes, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr1.0}.pdf}}
        \subfloat[Mercedes, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.5}.pdf}}
        \subfloat[Mercedes, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.1}.pdf}} \\
        \subfloat[Community, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr1.0}.pdf}}
        \subfloat[Community, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr0.5}.pdf}}
        \subfloat[Community, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr0.1}.pdf}}\\
        %\subfloat[Avg. LR, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr1.0_avglr}.pdf}}
        %\subfloat[Avg. LR, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.5_avglr}.pdf}}
        %\subfloat[Avg. LR, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.1_avglr}.pdf}}\\
        %\subfloat[Prune Rate, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr1.0_prrt}.pdf}}
        %\subfloat[Prune Rate, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.5_prrt}.pdf}}
        %\subfloat[Prune Rate, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.1_prrt}.pdf}}
        \caption{The predictive performance, measured by $R^2$, on the regression tasks.
        			The results from Mercedes-Benz dataset are on the top row, and the Community-Crime on the bottom row. 
			  The y-axis is aligned for each dataset (row) for ease of comparison across learning rates.
			%For the Community-Crime dataset, the predictive performances of the other models do not degrade much as in the Friedman and Mercedes-Benz datasets. 
			%We believe the relationship between features and target is more deterministic, and less likely to overfit. 
			%Still, we can observe PaloBoost outperforms the other models for both datasets.
    }
    \label{fig:regression}
\end{figure*}


\subsection{Regression Tasks}

The four SGTB models are evaluated on two publicly available regression datasets, the Mercedes-Benz Greener Manufacturing Dataset and the Communities Crime Dataset.
While only the coefficient of determination ($R^2$) results are presented, the results from our extensive experimental studies on adaptive learning rate and prune rate are available on the PaloBoost package webpage.

\subsubsection{Mercedes-Benz Greener Manufacturing Dataset}
Daimler, the parent company of Mercedes-Benz, performs exhaustive tests on its pre-release cars for the safety and reliability.
The process can easily consume a substantial amount of gas and time, and generate a large volume of carbon dioxide.
In the effort to reduce the testing time and conserve the environment, 
the company released its dataset that contains various measurements (features) and time to finish the test (target) through the Kaggle platform\footnote{https://www.kaggle.com/c/mercedes-benz-greener-manufacturing}.
As summarized in Table \ref{tab:data}, the dataset has only 4,209 samples with 460 features (post-processed). 
Thus, many complex models are likely to overfit on the small training sample and need to properly address the curse of dimensionality \cite{Trunk:1979, Hughes:1968}.

%\begin{figure*}
%    \centering
%        \subfloat[$R^2$, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr1.0}.pdf}}
%        \subfloat[$R^2$, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.5}.pdf}}
%        \subfloat[$R^2$, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.1}.pdf}} \\
        %\subfloat[Avg. LR, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr1.0_avglr}.pdf}}
        %\subfloat[Avg. LR, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.5_avglr}.pdf}}
        %\subfloat[Avg. LR, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.1_avglr}.pdf}}\\
        %\subfloat[Prune Rate, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr1.0_prrt}.pdf}}
        %\subfloat[Prune Rate, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.5_prrt}.pdf}}
        %\subfloat[Prune Rate, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_mercedes_ss0.7_lr0.1_prrt}.pdf}}
%        \caption{Mercedes-Benz Dataset [REG]. PaloBoost outperforms the other SGTB implementations. 
%        		The average learning rate for $\nu_{max}=0.1$ quickly converges to much smaller learning rates ($\approx 0.03$) after 30 iterations.}
%    \label{fig:mercedes}
%\end{figure*}

The top row in Figure~\ref{fig:regression} shows the predictive performance ($R^2$) on the Mercedes-Benz dataset.
Similar to the simulation results (Figure \ref{fig:friedman-perf}), PaloBoost achieves the best and most stable performance.
More impressively, PaloBoost suffers minimal degradation at the high learning rate ($\nu_{max} = 1.0$), while a noticeable decay occurs immediately for the other three models.
Furthermore, the performance differences across the three learning rates is marginal for PaloBoost, which demonstrates the robustness to the maximum learning rate parameter setting.
Unlike the other SGTB implementations that use a fixed learning rate, we observed that the average learning rate in PaloBoost dropped after a few iterations.
Moreover, approximately 40\% of the regions were pruned during the gradient-aware prune mechanism.
Together, these modifications contribute to the robust performance of PaloBoost.


\subsubsection{Communities and Crime Dataset}
Communities that have similar socioeconomic and law enforcement profiles may also experience similar types of crimes. 
Such information can be shared across police departments to enable cooperation.
In the effort to make such a data-driven system, 
Redmond \cite{Redmond:2002} created a dataset by combining three data sources: US Census in 1990, US FBI Uniform Crime Report in 1995, and 1990 US Law Enforcement Management and Administrative Statistics Survey.
The dataset, available on the UCI Repository\footnote{http://archive.ics.uci.edu/ml/datasets/communities+and+crime}, contains 127 features that include the percent of unemployed, percent under poverty, median income, etc. and the violent crime rate of community (numeric target).
This dataset contains only 1,994 samples with 127 features and has missing values (see Table \ref{tab:data}), therefore Scikit-Learn is omitted as a baseline.
The author of the dataset has stated that it has been carefully curated with only features that have plausible connection to crime.

%\begin{figure*}
%    \centering
%        \subfloat[$R^2$, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr1.0}.pdf}}
%        \subfloat[$R^2$, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr0.5}.pdf}}
%        \subfloat[$R^2$, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr0.1}.pdf}}\\
        %\subfloat[Avg. LR, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr1.0_avglr}.pdf}}
        %\subfloat[Avg. LR, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr0.5_avglr}.pdf}}
        %\subfloat[Avg. LR, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr0.1_avglr}.pdf}}\\
        %\subfloat[Prune Rate, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr1.0_prrt}.pdf}}
        %\subfloat[Prune Rate, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr0.5_prrt}.pdf}}
        %\subfloat[Prune Rate, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{reg_communities_ss0.7_lr0.1_prrt}.pdf}}
%        \caption{Communities Crime Dataset [REG]. Unlike the Friedman and Mercedes datasets, the predictive performances of the other models do not degrade much as they iterate more. We believe the relationship between features and target is more deterministic, and less likely to overfit. Still, PaloBoost outperforms the other models.}
%    \label{fig:crime}
%\end{figure*}

The bottom row in Figure~\ref{fig:regression} illustrates the results from the Communities and Crime Dataset experiments. 
As can be seen, PaloBoost exhibits the most stable behavior across many iterations.
However, unlike the previous two datasets (Mercedes-Benz and simulated), the performance of the benchmark models do not suffer a significant degradation.
Since the feature selection has already been done by the author, the features are not noisy, thereby mitigating the curse of dimensionality.
While PaloBoost does not obtain the highest $R^2$ overall compared to XGBoost, we note that the values between the different learning rates is much smaller in comparison. 
This eliminates the need to finely tune the learning rate and the number of iterations.



\subsection{Classification Tasks}

Next, we present the various SGTB models on four different classification tasks: Amazon Employee Access, Pulsar Detection, Carvana, and BNP-Paribas.
Although we only present the predictive performance (AUROC), the adaptive learning rate and prune rate results are available on the PaloBoost package webpage.

\begin{figure*}
    \centering
        \subfloat[Amazon, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr1.0}.pdf}}
        \subfloat[Amazon, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr0.5}.pdf}}
        \subfloat[Amazon, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr0.1}.pdf}}\\[-2ex]
        \subfloat[Pulsar, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr1.0}.pdf}}
        \subfloat[Pulsar, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr0.5}.pdf}}
        \subfloat[Pulsar $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr0.1}.pdf}}\\[-2ex]
        \subfloat[Carvana, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr1.0}.pdf}}
        \subfloat[Carvana, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr0.5}.pdf}}
        \subfloat[Carvana, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr0.1}.pdf}}\\[-2ex]    
        \subfloat[BNP, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr1.0}.pdf}}
        \subfloat[BNP, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr0.5}.pdf}}
        \subfloat[BNP, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr0.1}.pdf}}
        \caption{
        Predictive performance, measured in AUROC, for the four classification tasks.
        From the top, at each row, we have Amazon Employee Access Dataset (1st row),  Pulsar Detection Dataset (2nd row), Carvana Dataset (3rd row), and BNP-Paribas Cardif Dataset (4th row).
        The y-axis is aligned for each dataset (row) for ease of comparison across learning rates.
        }
        %For the Amazon dataset, PaloBoost is slower to converge, showing poorer performance than the other models. 
        %Still, PaloBoost shows comparable performances for higher learning rates.
	%For all the datasets. PaloBoost does not show any performance degradation even for higher learning rates. 
        %The other models show overfitting behaviors even for smaller learning rates.}
    \label{fig:classification}
\end{figure*}



\subsubsection{Amazon Employee Access Dataset}
Depending on their roles, Amazon's employees have different access rights on their internal web resources.
Supervisors often spend a considerable amount of time manually granting and revoking the access rights of their employees.
To automate this process and increase the overall work efficiency,
Amazon released its historical employee access dataset on Kaggle\footnote{https://www.kaggle.com/c/amazon-employee-access-challenge} that contains employee attributes, resource ID, and whether the access was granted or not (target).
Interestingly, the dataset only contains eight categorical features (preprocessed to 115 features) for 32,769 employees (see Table \ref{tab:data}).
Also, many top-scoring solutions on the Kaggle leaderboard noted the importance of capturing the interaction between categorical features to improve the predictive performance.
This is due to the fact that the employees access rights are somewhat well defined given a specific configuration of employee attributes.
Therefore, there exists a fairly deterministic relationships between the features and the target, which can be obtained by a highly customized preprocessing step.
However, performance improvement is not the key objective of our experiments, so minimal preprocessing is performed.


%\begin{figure*}
 %   \centering
 %       \subfloat[AUROC, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr1.0}.pdf}}
 %       \subfloat[AUROC, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr0.5}.pdf}}
 %       \subfloat[AUROC, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr0.1}.pdf}}\\    
        %\subfloat[Avg. LR, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr1.0_avglr}.pdf}}
        %\subfloat[Avg. LR, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr0.5_avglr}.pdf}}
        %\subfloat[Avg. LR, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr0.1_avglr}.pdf}}\\
        %\subfloat[Prune Rate, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr1.0_prrt}.pdf}}
        %\subfloat[Prune Rate, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr0.5_prrt}.pdf}}
        %\subfloat[Prune Rate, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_amazon_ss0.7_lr0.1_prrt}.pdf}}
 %       \caption{Amazon Employee Access Dataset [CLS]. 
%        	PaloBoost is slower to converge, showing poorer performance than the other models. 
%        We believe the dataset is less likely to overfit. 
%        In fact, higher learning rates provide comparable (or better) performance with lower learning rates for all models.}
%    \label{fig:amazon}
%\end{figure*}

The top most row in Figure~\ref{fig:classification} presents the results from the Amazon Employee Dataset experiment.
Unlike the previous datasets (simulated, Mercedes-Benz, and Crime), the AUROC of PaloBoost, SGTB-Bonsai, and XGBoost are still improving after 200 iterations.
Only Scikit-Learn demonstrate overfitting on the dataset.
We suspect there are two reasons for this behavior.
Since all the features in this dataset are categorical, the degree of freedom in the input space is finite, thereby reducing the risk of the curse of dimensionality.
Secondly, the fairly deterministic nature of the features and the targets combined with the large sample size make it less prone to overfitting.

Another important observation from Figure \ref{fig:classification} is that PaloBoost converges slower compared to the other models on this dataset.
This is because PaloBoost has two additional regularization mechanisms: gradient-aware pruning and adaptive learning rates.
While these modifications are likely to improve the performance for a complex problem (e.g., large number of features, small dataset size, large amount of noise, etc.), it can hinder the performance on simpler problems.
By regularizing the trees and the learning rates, PaloBoost is unable to quickly learn an appropriate model and thereby requires more iterations to achieve the same accuracy\footnote{PaloBoost eventually achieves comparable AUROC.}.
Therefore, PaloBoost may not be appropriate when standard SGTB models are not prone to overfitting.

\subsubsection{Pulsar Detection Dataset}
Pulsars, rapidly rotating neutron stars, are known to emit a detectable pattern of electromagnetic radiation.
Unfortunately, automated detection based on the pattern is often a non-trivial task due to radio frequency interference and noise.
Nowadays, machine learning techniques are adopted to extract candidates for detecting pulsars.
In the effort to develop such machine learning detection algorithms, 
Lyon curated and published the HTRU2 (High Time Resolution Universe Survey - South) dataset \cite{Lyon:2016, Lyon:data}.
The dataset, published on UCI\footnote{https://archive.ics.uci.edu/ml/datasets/HTRU2}, contains the profiles of electromagnetic waves and the label (pulsar or not) of 17,898 examples, 
where 1,639 examples are pulsars (positive class). 
All eight features are numeric and have no missing values (see Table \ref{tab:data}).

%\begin{figure*}
%    \centering
 %       \subfloat[AUROC, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr1.0}.pdf}}
%        \subfloat[AUROC, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr0.5}.pdf}}
%        \subfloat[AUROC, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr0.1}.pdf}}\\
        %\subfloat[Avg. LR, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr1.0_avglr}.pdf}}
        %\subfloat[Avg. LR, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr0.5_avglr}.pdf}}
        %\subfloat[Avg. LR, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr0.1_avglr}.pdf}}\\
        %\subfloat[Prune Rate, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr1.0_prrt}.pdf}}
        %\subfloat[Prune Rate, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr0.5_prrt}.pdf}}
        %\subfloat[Prune Rate, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_htru_ss0.7_lr0.1_prrt}.pdf}}
%        \caption{Pulsar Detection Dataset [CLS]. PaloBoost exhibits the most stable performances. 
%        		AUROC values are overall very high, indicating the problem is relatively easy.
%		However, the other models quickly overfit to the training samples when their learning rates are high.}
%    \label{fig:pulsar}
%\end{figure*}

The second row in Figure~\ref{fig:classification} illustrates the results from the Pulsar Detection Dataset experiment.
As can be seen, PaloBoost exhibits the most stable and best performance overall.
However, the performance differences are practically indistinguishable for smaller learning rates.
This maybe a result of the dataset curation process, where only engineered features that are strongly correlated with the target variable were included.
Even a single, albiet highly customized, decision tree algorithm could achieve a reasonable performance \cite{Lyon:2016}. 
In other words, the dataset has no noisy features, thus overfitting is less likely to happen even for complex models.

\subsubsection{Carvana Dataset}

When auto dealers purchase used cars from an auction, 
there is a risk of purchasing cars with serious issues such as tampered odometers and mechanical issues, 
which is commonly referred as ``kicks`` in the industry.
Carvana is an online used-car dealers company. 
The company released its dataset on Kaggle\footnote{https://www.kaggle.com/c/DontGetKicked} that contains used cars' attributes, such as make, model, vehicle age, odometer, etc., and the target variable (kick or not). 
The dataset (summarized in Table \ref{tab:data}) has 72,983 samples, with 151 numeric features (after preprocessing).
Due to missing values, Scikit-Learn is omitted from this experimental study.

%\begin{figure*}
%    \centering
%        \subfloat[AUROC, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr1.0}.pdf}}
%        \subfloat[AUROC, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr0.5}.pdf}}
%        \subfloat[AUROC, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr0.1}.pdf}}\\    
        %\subfloat[Avg. LR, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr1.0_avglr}.pdf}}
        %\subfloat[Avg. LR, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr0.5_avglr}.pdf}}
        %\subfloat[Avg. LR, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr0.1_avglr}.pdf}}\\
        %\subfloat[Prune Rate, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr1.0_prrt}.pdf}}
        %\subfloat[Prune Rate, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr0.5_prrt}.pdf}}
        %\subfloat[Prune Rate, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_carvana_ss0.7_lr0.1_prrt}.pdf}}
%        \caption{Carvana Dataset [CLS]. PaloBoost does not show any performance degradation even for higher learning rates. 
%        The other models show overfitting behaviors even for smaller learning rates. 
%        The average learning rates for PaloBoost nicely attenuates as PaloBoost iterates, preventing the algorithm to overfit. }
%    \label{fig:carvana}
%\end{figure*}

The third row in Figure~\ref{fig:classification} shows the results from the dataset.
As can be seen, the two baseline models clearly display overfitting behaviors for all three learning rates.
Moreover, the dataset is prone to overfitting, as illustrated by the Kaggle leaderboards.
A comparison of the public and private leaderboards\footnote{Kaggle sets one third of test data for ranking the public leaderboard, and the rest for the private leaderboard. The private leaderboard is closed during the competition, and announced after the competition is closed. This is to prevent the overfitting on the test set \cite{Blum:2015}.} shows considerable movement between the top 4 teams. 
This indicates the top teams' models likely suffered from overfitting.
Notably, PaloBoost exhibits extremely stable predictive performances and records the best scores for all cases.
Moreover, the difference in performance across the three learning rates is almost negligible.
Although not shown, the prune and adaptive learning rates displayed similar patterns to the simulated dataset (Figure \ref{fig:friedman-palo}).


\subsubsection{BNP Paribas Cardif Claims Dataset}

Insurance claim payments involve many levels of manual checks, sometimes requires more information to be collected, 
and can take a substantial amount of time till the final payments.
Some of these claims, however, can be processed much faster with machine learning techniques.
BNP Paribas Cardif, one of the largest personal insurance company, released some of its data via the Kaggle platform\footnote{https://www.kaggle.com/c/bnp-paribas-cardif-claims-management}
that contains various claim attributes (features) and if the claim's approval could be accelerated or not (target).
The dataset consists of 114,321 samples with 273 numeric features (after preprocessing).
Scikit-Learn is omitted from this study as the dataset has many missing values (see Table \ref{tab:data}).
This dataset contains the largest number of samples (of the seven datasets) and shows a fair degree of complexity. 

%\begin{figure*}
%    \centering
%        \subfloat[AUROC, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr1.0}.pdf}}
%        \subfloat[AUROC, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr0.5}.pdf}}
%        \subfloat[AUROC, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr0.1}.pdf}}\\
        %\subfloat[Avg. LR, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr1.0_avglr}.pdf}}
        %\subfloat[Avg. LR, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr0.5_avglr}.pdf}}
        %\subfloat[Avg. LR, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr0.1_avglr}.pdf}}\\
        %\subfloat[Prune Rate, $\nu_{max}=1.0$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr1.0_prrt}.pdf}}
        %\subfloat[Prune Rate, $\nu_{max}=0.5$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr0.5_prrt}.pdf}}
        %\subfloat[Prune Rate, $\nu_{max}=0.1$]{\includegraphics[width=0.33\textwidth]{figures/{cls_bnp_ss0.7_lr0.1_prrt}.pdf}}
 %       \caption{BNP-Paribas Cardif Dataset [CLS]. For higher learning rates, even PaloBoost shows some degree of overfitting, however, the level of performance degradation is much less than the other models.
%        The average learning rates for PaloBoost adaptively decrease over iterations.
%        PaloBoost shows the best and stable performances for all cases.}
%    \label{fig:bnp}
%\end{figure*}

The last row in Figure~\ref{fig:classification} illustrates the results from the BNP Paribas Cardif Claims Dataset experiment.
Similar to all but the Amazon classification task, PaloBoost offers the most stable and best predictive performance.
The competitors involved in this Kaggle challenge remarked that they suspect the dataset has additional noise to the features\footnote{See discussions 19240 and 20247 on the Kaggle discussion board at \url{https://www.kaggle.com/c/bnp-paribas-cardif-claims-management/discussion/} as some examples.}.
Many winning solutions were based on extensive feature engineerings, identifying the relationships of the features, and removing the noisy features.
The impressive performance from PaloBoost suggests the ability to effectively identify the noisy features to yield a more robust model.
This also suggests that PaloBoost can outperform other SGTB implementations when a minimal preprocessing is applied to a noisy dataset.

Based on our extensive experiments, PaloBoost outperforms existing SGTB models when a dataset has many noisy features and is prone to overfitting.
While PaloBoost is not guaranteed to achieve the best predictive performance on all datasets (see the Amazon results in the top row of Figure \ref{fig:classification}), it is less prone to overfitting.
From Figures \ref{fig:friedman-perf}, \ref{fig:regression}, and \ref{fig:classification}), we observe that PaloBoost exhibits a gradual performance degradation in all seven datasets, unlike the other baseline models.
Moreover, the predictive performance of PaloBoost using different learning rates is relatively small.
Thus, we conclude that PaloBoost is robust to the specification of the learning rate ($\nu_{max}$), the tree depth, and also the number of iterations $M$.















==> bk/_pb-introduction_v1.tex <==
\section{Introduction}

Stochastic Gradient TreeBoost (SGTB) is one of the most widely used off-the-shelf machine learning algorithms \cite{Bekkerman:2015, He:2014, Chen:2016ga, Friedman:2006}.
SGTB is a stage-wise additive model where the base trees are fitted to the subsampled gradients (or errors) at each stage \cite{Friedman:2001ue, Friedman:2002ex}. 
The randomness introduced by subsampling speeds up the computation time and mitigates overfitting.
Consequently, SGTB can provide robust performance over various classification, regression, and even ranking tasks \cite{Burges:2010, Li:2008}.
Many empirical results have demonstrated SGTB's ability to model complex and large data relatively fast and accurately.
Furthermore, the effectiveness and pervasiveness of SGBT can be found in many winning solutions in public data science challenges \cite{Chen:2016ga}.

%Stochastic Gradient TreeBoost (SGTB) is a stage-wise additive model where its base trees are fitted to the subsampled gradients (or errors) at each stage
%Many empirical results illustrate that it can model very complex and large data relatively fast and accurately.
%Moreover, it can provide robust performance over various classification and regression tasks \cite{}.
%Due to these advantages, SGTB has been one of the most widely used off-the-shelf machine learning algorithms.
%Many winning solutions in public data science challenges attest both the effectiveness and wide adoption of SGTB \cite{Chen:2016ga}.

In many cases, SGTB can provide reasonable performance with default parameter settings.
However, to achieve its best performance, extensive parameter tuning is usually required.
These parameters are mainly 1) max depth of trees, 2) number of trees, and 3) learning rate.
Having deeper trees and more trees can reduce training errors more rapidly, while these may increase the chance of overfitting \cite{Friedman:2001ue, Ridgeway:2012wr}.
Lower learning rates can slow down this aggressive fitting to the training data at each stage, 
but more trees are needed to reach to a similar level of performance \cite{Ridgeway:2012wr}. 
As can be seen, balancing between overfitting and best performance can be more of an art than a science in practice.

This delicate parameter tuning can be a bottleneck for many time-sensitive or performance-critical practical applications.
An ideal boosting algorithm would converge faster with less trees, achieving its best performance without overfitting.
The learning rate of such a boosting algorithm would dynamically adjust to 
higher when it needs to converge faster, and lower when it is approaching its best performance.
The max depth of trees would change dynamically, and the number of trees will be less overall.
The question is: Can we build such an ideal boosting algorithm?

In an attempt to design such an algorithm, we present PaloBoost, a boosting algorithm that is easier to tune parameters and can potentially achieve better performance.
PaloBoost extends SGTB using two \textit{out-of-bag sample} regularization techniques: 1) Gradient-aware Pruning and 2) Adaptive Learning Rate.
Out-of-bag (OOB) samples are the samples not included in subsampling, and commonly available in many subsampling-based algorithms \cite{Breiman:1996, Breiman:2001}.
In boosting algorithms, OOB errors, the errors estimated from OOB samples, are used as computationally cheaper alternatives for cross-validation errors \cite{Ridgeway:2012wr}.
These error estimates are typically used to determine the number of trees - also known as early stopping \cite{Ridgeway:2012wr}.
Simply speaking, in SGTB, OOB samples play merely a third-party observer role in the overall training process.
The algorithm tracks OOB errors, but the errors never affect the remaining training process other than early stopping.

PaloBoost, on the other hand, treats OOB samples as a second batch of training samples for adjusting learning rate and max tree depth.
At each stage of PaloBoost, we take OOB samples, and check if the OOB errors will decrease with a given tree size and learning rate.
If the OOB error is not decreasing, it means that the tree is too specific and failed to generalize to the dataset.
We prune the tree leaves, so that OOB errors are controlled.
Next, we find optimal learning rates that will decrease the OOB errors the most, and repeat this entire process at each stage.
In short, PaloBoost randomly partitions training samples into two sets at each stage: one for leaning a tree structure, and the other for pruning and adjusting learning rates. 

This two-stage training process frequently appear in many machine learning algorithms, 
when we need to estimate two distinct sets of parameters or models.
Among many examples \cite{Zhang:2018, Romero:2015, Barshan:2015}, we find that hyperparameter tuning is the most relevant.
In hyperparameter tuning \cite{Efron:1983, Kohavi:1995}, 
we sequentially estimate parameters from two disjoint datasets - 
1) regular parameters from a training set and 2) hyperparameters from a validation set.
In PaloBoost, this translates to 1) in-bag samples for growing trees and 2) out-of-bag samples for pruning and adjusting learning rates.
The main difference is that PaloBoost's hyperparameter tuning happens at each stage with different out-of-bag samples.

We compare the performance of PaloBoost with various open-source SGTB implementations such as Scikit-Learn \cite{scikit-learn} and XGBoost \cite{Chen:2016ga}.
Our benchmark datasets include one simulated data \cite{Friedman:1991} and six real datasets from Kaggle \cite{kaggle} and UCI repositories \cite{Dua:2017}.
From the experiments, we observe that PaloBoost shows gradually and adaptively decreasing learning rates and tree depths over its iterations.
This adaptive mechanism makes PaloBoost robust to overfitting and perform better than other SGTB implementations in many cases.


==> bk/_pb-paloboost_v1.tex <==

\section{PaloBoost}\label{sec:paloboost}

To achieve its best performance, SGTB needs to tune its hyperparameters - they are learning rate, number of trees, and depth of trees. 
However, they are closely related each other making the tuning process quite difficult.
For example, a learning rate and a number of trees are in a trade-off relationship, known as  the $\nu$-$M$ trade-off \cite{Friedman:2001ue, Friedman:2002ex}.
Lower learning rates ($\nu$) may result in better performance, but more number of trees ($M$) are usually required to achieve a similar level of performance. 
Typically, we set aside a set of unseen samples, a validation set, and use the dataset to tune these hyperparameters.

We illustrate how this process works with a one-stage SGTB model i.e. $M=1$. 
To tune the tree depth and learning rate, we first partition a dataset into three sets: training, validation, and test.
We will use the test set to estimate the expected performance, so it will not be used in any (hyper)parameter tuning.
The first step is to fit the intercept term, $F_0$, using the training set.
Next, we randomly subsample data points from the training set, and fit a tree on those sampled gradients.
We measure the performance on the validation set for a given learning rate and tree depth.
We repeat this process multiple times by varying learning rate and tree depth, and pick the hyperparameters with the best performance.
The same principle applies for more complex SGTBs with multiple stages - 1) fit a SGTB on the training set, 2) monitor the performance with the validation set, and 3) repeat multiple times varying hyperparameters.

As can be seen, the tuning process is straightforward. 
However, it is also easy to see that the whole cycle can consume a substantial amount of time and computing resources.
Making things worse, in many practical applications,
the best-tuned hyperparameters may not produce the best results in real testing environments. 
This is because the test samples are usually drawn from a slightly different distribution from the training samples - 
note that there is a fine line between the best performance and overfitting. 
This sometimes makes the computationally expensive hyperparameter tuning less appealing.
The development of PaloBoost is motivated by this line of complications. 

\begin{figure}
    \centering
        \includegraphics[width=1.0\columnwidth]{figures/paloboost-diagram.pdf}
        \caption{Data flows in SGTB and PaloBoost.}
    \label{fig:dataflow}
\end{figure}

Our goal is to design a variant of SGTB that is less sensitive to hyperparameters, yet is able to produce robust performance.
We believe there are many different approaches for such a goal.
In our case, we found a clue in our one-stage SGTB example and its \textit{under-utilized} out-of-bag (OOB) samples.
Both validation and OOB samples are not seen during the training phase.
Thus, we can simply use the OOB samples to tune the hyperparameters.
This may sound still the same as SGTB, but
becomes quite different as we move to multi-stages ($M>1$).
In the next stage, we will fit a new tree to the subsampled gradients.
Recall that we used OOB samples to tune learning rate and tree depth. 
Although we have different OOB samples from the previous stage, 
we apply the same principle, using the OOB samples to find the optimal learning rate and tree depth.
This will be most likely different from the previous stage, but this is, in fact, the core idea of PaloBoost.
PaloBoost is a variant of SGTB that has adaptive learning rates and tree depths.
We repeat this process over and over till we reach the $M$th stage.
Figure~\ref{fig:dataflow} illustrates the data flow differences in SGTB and PaloBoost.

The learning rate and tree depth in PaloBoost are not hyperparameters any more.
They are, technically, another set of parameters that are estimated over the course of training. 
The downside of this new approach is, of course, computational overhead caused by estimating new parameters. 
When we were designing PaloBoost, we assumed that line search at every stage is not feasible.
We needed to develop smarter approaches to avoid expensive computations.
The next subsections will discuss how we can determine tree depths and learning rates in a faster way.

\subsection{Rate-dependent Pruning}

Many SGTB implementations have a parameter to set the max depth of trees. 
We wanted to make PaloBoost not too much different from other SGTBs, while having more flexible tree depths.
Thus, we decided to use a pruning technique using OOB samples, which we call Rate-dependent Pruning.

Rate-dependent Pruning works as follows. 
After a tree is fitted to subsampled gradients, 
we apply the tree on OOB samples.
For each disjoint region of the OOB samples, 
we test if the loss is actually reduced on the OOB samples by adding the new leaf estimate:
\begin{equation}
\sum_{i}^{L_j} \text{Loss}(y_i, \hat{y}_i) > \sum_{i}^{L_j} \text{Loss}(y_i, \hat{y}_i + \nu_{max} \gamma_j)
\label{eq:prune}
\end{equation}
where the leaf estimate is the gradient multiplied by the learning rate.
If the loss is not reduced, then we roll up the branch.
This process is summarized in Algorithm~\ref{algo:prune}.

\begin{algorithm}
\DontPrintSemicolon
$\{(R_j, R_k)\} = \text{Find-Sibling-Pairs}(\{R_j\}_{j=1}^J)$\;
\For{each sibling pair in $\{(R_j, R_k)\}$}{
	$\{y_i, \mathbf{x}_i\}_1^{L_j} = \text{Out-of-Bag}(\{y_i, \mathbf{x}_i\}_1^{N} | R_j)$\;
	$\{y_i, \mathbf{x}_i\}_1^{L_k} = \text{Out-of-Bag}(\{y_i, \mathbf{x}_i\}_1^{N} | R_k)$\;	
	\uIf{$\sum_{i}^{L_j} \text{Loss}(y_i, \hat{y}_i) < \sum_{i}^{L_j} \text{Loss}(y_i, \hat{y}_i + \nu_{max} \gamma_j)$}{
		do\_merge = True\;		
	}\uElseIf{$\sum_{i}^{L_k} \text{Loss}(y_i, \hat{y}_i) < \sum_{i}^{L_k} \text{Loss}(y_i, \hat{y}_i + \nu_{max} \gamma_k)$}{
		do\_merge = True\;			
	}\Else{ 
		do\_merge = False\; 
	}
	\If{do\_merge}{
		Merge($R_j$, $R_k$)
	}
}
\caption{Rate-Dependent Pruning}
\label{algo:prune}
\end{algorithm}

Rate-dependent Pruning has roots in a bottom-up ``reduced-error pruning`` in the decision tree literature.
In the reduced-error pruning, we compare the errors on OOB samples between children and parent nodes.
If the children nodes do not decrease the OOB errors, then we roll up the branch.
In boosting, however, this approach ignores two important aspects: previous trees and learning rate. 
Trees in boosting are dependent each other, and the node estimates are always multiplied by the learning rate.
For this reason, we needed a new pruning approach.

A rationale for Rate-Depenent Pruning is related to sample sizes per node.
As we split more, the sample size per node becomes smaller.
Smaller sample sizes result in higher variances of the node estimates $\gamma$, which is also likely to increase generalization errors.
Furthermore, our adaptive learning rate mechanism, which we will illustrate in the next section, produce more stable results with larger samples. 
In some sense, Rate-dependent Pruning serves as a preprocessing step for the adaptive learning rate mechanism.

\subsection{Adaptive Learning Rate}

Learning rate is typically optimized through line search. 
There is no easy solution even if we focus on one-stage boosting.
Our original idea is to find different learning rates at each stage of boosting.
Performing line search at every stage may create substantial computational overhead.
We needed a different framework for learning rate that does not require line search.
Interestingly enough, we found our solution in a more complex setting.
Different learning rates at each stage are difficult to calculate, but different learning rates at ``each stage and each region`` were much easier to estimate - even with closed form solutions.

Adaptive Learning Rates in PaloBoost are not just different learning rates at each stage. 
We are estimating a multiplicative factor that optimizes the OOB loss per each disjoint region at each stage. 
The benefit of this approach is that we have closed form solutions for many loss functions.
For example, a learning rate for the negative binomial log-likelihood loss function can be obtained by solving the following equation:
\begin{equation} 
\nu_j^* = \argmax_\nu \sum_{i}^{L_j} y_i (\hat{y}_i + \nu\gamma_j) - \log(1+\text{exp}(\hat{y}_i + \nu\gamma_j))
\end{equation}
where $L_j$ represents the number of samples in the leaf of interest. 
We have a closed for solution:
\begin{equation}
\nu_j =  \log(\frac{\sum_{i}^{L_j} y_i }{ \sum_{i}^{L_j} (1-y_i)\text{exp}(\hat{y}_i)})/\gamma_j
\end{equation}
Similarly for a squared error function, we have:
\begin{equation} 
\nu_j^* = \argmax_\nu \sum_{i}^{L_j} (y_i - (\hat{y}_i + \nu\gamma_j))^2 
\end{equation}
where its closed form solution is give as:
\begin{equation}
\nu_j =  \frac{\sum_{i=1}^{L_j}(y_i - \hat{y}_i) }{ \gamma_j L_j}
\end{equation}

Algorithm~\ref{algo:alr} illustrates our adaptive learning rate strategy. 
As can be seen, we added a clipping function on the estimated learning rate.
This is because the estimated learning rates are usually based on small sample sizes, 
and the values can fluctuate in a wide range.
In practice, we observed several cases where the estimates are negative or even above one.
To enforce stability, and also maintain similarity with the usages of the original SGTB implementations,
we post-process the estimated learning rates with the maximum learning rate parameter, $\nu_{max}$.
As a result, the effective learning rate per region per stage ranges between zero and the maximum learning rate.

\begin{algorithm}
\DontPrintSemicolon
$\{(R_j, R_k)\} = \text{Find-Sibling-Pairs}(\{R_j\}_{j=1}^J)$\;
\For{$R_j$ in $\{R_j\}_{j=1}^J$}{
	$\{y_i, \mathbf{x}_i\}_1^{L_j} = \text{Out-of-Bag}(\{y_i, \mathbf{x}_i\}_1^{N} | R_j)$\;
	\uIf{distribution==``gaussian``}{
		$\nu_j =  \text{clip}(\frac{\sum_{i=1}^{L_j}(y_i - \hat{y}_i) }{ \gamma_j L_j}, 0, \nu_{max})$\;		
	}\ElseIf{distribution==``bernoulli``}{
		$\nu_j = \text{clip}( \log(\frac{\sum_{i}^{L_j} y_i }{ \sum_{i}^{L_j} (1-y_i)\text{exp}(\hat{y}_i)})/\gamma_j , 0, \nu_{max})$\;	
	}
}
\caption{Adaptive Learning Rate with Out-of-Bag Loss Reduction}
\label{algo:alr}
\end{algorithm}

\subsection{Implementation}

PaloBoost adds the Rate-dependent Pruning and Adaptive Learning Rate to the original SGTB algorithm.
Algorithm~\ref{algo:paloboost} illustrates the details of PaloBoost.
We implemented PaloBoost using the Bonsai Decision Tree framework \cite{bonsai-dt}.
The Bonsai framework allows easy manipulation of decision trees.
The framework are written mostly in Python, and its core computation modules are written in Cython.

\begin{algorithm}
\DontPrintSemicolon
$F_0 = \argmin_{\beta} \sum_{i=1}^N L(y_i, \beta)$\;
\For{$m \gets 1$ \textbf{to} $M$}{
	$\{y_i, \mathbf{x}_i\}_1^{N^\prime} = \text{Subsample}(\{y_i, \mathbf{x}_i\}_1^{N}, \text{rate}=q)$\;
	$z_i = -\frac{\partial}{\partial F(\mathbf{x}_i)} L(y_i, F(\mathbf{x}_i)) \Bigr|_{F=F_{m-1}}$, for $i=1, \cdots, N^\prime$\;
	$\{R_{jm}\}_1^J = \text{XGB-RegressionTree}(\{z_i, \mathbf{x}_i\}_i^{N^\prime})$\;
	$\gamma_{jm} = \argmin_{\gamma} \sum_{\mathbf{x}_i \in R_{jm}} L(y_i, F_{m-1}(\mathbf{x}_i) + \gamma)$, for $j=1, \cdots, J$ \;
	$\{R_{jm}, \gamma_{jm}\}_1^{J^\prime} = \text{Rate-Dependent-Pruning}(\{R_{jm}, \gamma_{jm}\}_1^J, \nu_{max})$\;
	$\nu_{jm} = \text{Learning-Rate-Adjustment}(\gamma_{jm}, \nu_{max})$, for $j=1, \cdots, J^\prime$\;
	$F_m(\mathbf{x}) =F_{m-1}(\mathbf{x}) +   \sum_{j=1}^J \nu_{jm} \gamma_{jm} \mathbbm{1}(\mathbf{x} \in R_{jm})$\;
}
\caption{PaloBoost}
\label{algo:paloboost}
\end{algorithm}

Although PaloBoost has more parameters to estimate than regular SGTB algorithms, but 
its training speed is not so much slower than the regular SGTB's training speed.
We measured the training speeds of 1) PaloBoost,  2) SGTB implemented in Bonsai, 3) Scikit-Learn, and 4) XGBoost. 
Figure~\ref{fig:speed} shows the measured training time over simulated training sample sizes.
As can be seen, the performance of PaloBoost is comparable with the other implementations even for large sample sizes e.g. one million samples.

\begin{figure}
    \centering
        \includegraphics[width=0.8\columnwidth]{figures/{reg_friedman_ss0.7_lr0.1_speed}.pdf}
        \caption{Runtime}
    \label{fig:speed}
\end{figure}

\subsection{Modified Feature Importance}\label{sec:paloboost-feaures}

Traditionally, a feature importance in SGTB is calculated as the summation of squared error improvements by the feature \cite{Elith:2008}.
However, as Friedman noted \cite{bonsai-dt}, the measure is purely based on heuristic arguments.
In fact, the formula is adopted from RandomForest \cite{Breiman:2001}.

Although the traditional approach has proven useful in many applications, 
we noticed the formula for the feature importance ignores three important aspects of PaloBoost: 
leaf estimate, coverage of region, and adaptive learning rate. 
As seen in the SGTB algorithm, leaf estimates are recalibrated to minimize the loss function.
No matter how much improvement a feature has made at a particular branch, 
there is always a chance that the resultant leaves may have zero effects or very small coverage.
Furthermore, the adaptive learning rate may turn out to be zero with our Adaptive Learning Rate algorithm, 
in which case the feature has no contribution in prediction.

These issues led us create a new formula for PaloBoost's feature importances 
that capture these three quantities:
%\begin{equation}
%f_k =  \frac{\sum_{j=1}^{J} | R_j | | \gamma_j |  \mathbbm{1}(f_k \in \text{Rules}_j)}{J \sum_{j=1}^{J} | R_j | }
%\end{equation}
\begin{equation}
f_k = \sum_{m=1}^{M}  \frac{ \sum_{j=1}^{J_m} \nu_{jm} | R_{jm} |  | \gamma_{jm} |  \mathbbm{1}(f_k \in \text{Rules}_{jm})}{J_m \sum_{j=1}^{J} R_{jm}}
\end{equation}
where $|R_{jm}|$ represent the coverage of the region $R_{jm}$, 
and $\text{Rules}_{jm}$ denotes the logical rules that define the region $R_{jm}$.
For example, $\text{Rules}_{jm}$ may have a form of $(x_0 > 0.5 \text{ AND } x_1 < 1.0 \text{ AND } x_3 > -1)$, 
and in this case, $\mathbbm{1}(f_1 \in \text{Rules}_{jm})$ will be one as $x_1$ is in the rules.
In other words, the new feature importance first looks at each leaf, and see if a feature is used to define the leaf.
If used, then we multiply the size of region with the effective absolute node estimate, $\nu_{jm}|\gamma_{jm}|$. 
Finally, we sum over all the leaves and all the stages. 
In short, this new feature importance is leaf-centric, while the old feature importance is branch-centric.

